Robust Reward Modeling via Causal Rubrics

Reward models (RMs) are fundamental to aligning Large Language Models (LLMs) via human feedback, yet they often suffer from reward hacking. They tend to latch on to superficial or spurious attributes, such as response length or formatting, mistaking these cues learned from correlations in training data for the true causal drivers of quality (e.g., factuality, relevance). This occurs because standard training objectives struggle to disentangle these factors, leading to brittle RMs and misaligned policies. We introduce Crome (Causally Robust Reward Modeling), a novel framework grounded in an explicit causal model designed to mitigate reward hacking. Crome employs the following synthetic targeted augmentations during training: (1) Causal Augmentations, which are pairs that differ along specific causal attributes, to enforce sensitivity along each causal attribute individually, and (2) Neutral Augmentations, which are tie-label pairs varying primarily in spurious attributes, to enforce invariance along spurious attributes. Notably, our augmentations are produced without any knowledge of spurious factors, via answer interventions only along causal rubrics, that are identified by querying an oracle LLM. Empirically, Crome significantly outperforms standard baselines on RewardBench, improving average accuracy by up to 5.4% and achieving gains of up to 13.2% and 7.2% in specific categories. The robustness of Crome is further testified by the consistent gains obtained in a Best-of-N inference setting across increasing N, across various benchmarks, including the popular RewardBench (covering chat, chat-hard, safety, and reasoning tasks), the safety-focused WildGuardTest, and the reasoning-specific GSM8k.

==> archived/am_20250506.tex <==
\section{Methodology: Causal Data Augmentation for Robust Reward Modeling}
\label{sec:methodology}

Building upon the causal framework established in Section \ref{sec:preliminaries}, we introduce our methodology for training a robust reward model, $\hat{R}_\phi$. The central objective is to guide the model to learn preferences based on the true causal drivers of response quality ($C$) while remaining invariant to spurious attributes ($SP$). This is crucial because reliance on spurious attributes often leads to reward hacking, overfitting, and poor generalization to out-of-distribution prompts or response styles. Our approach achieves this by augmenting the standard preference dataset $\mathcal{D}_{pref}$ with synthetically generated examples $\mathcal{D}_{aug}$ designed to explicitly disentangle these factors.


Our approach consists of four sequential steps. First, we identify the relevant causal and potential spurious attributes for evaluating answers to a given query. Second, we leverage Large Language Models (LLMs) to generate counterfactual answer pairs that selectively manipulate these attributes. Third, we filter the generated data to ensure quality and focus on informative examples. Finally, we train the reward model $\hat{R}_\phi$ on the combined dataset using a modified pairwise preference loss function. We detail each step subsequently.

\subsection{Step 1: Attribute Identification}
\label{subsec:attribute_identification}

The foundation of our causal approach lies in identifying the attributes that genuinely determine answer quality versus those that are merely correlated with it. For a given query $Q$, potentially informed by example answers $(y_w, y_l)$ from $\mathcal{D}_{pref}$, we define two sets of attributes: \emph{Causal attributes} $C = (C_1, \dots, C_\ell)$, which fundamentally impact the ground-truth reward $R$ (e.g., \textit{factuality}, \textit{relevance}), and \emph{Spurious attributes} $SP = (SP_1, \dots, SP_k)$, which do not intrinsically affect $R$ but might influence preferences (e.g., \textit{verbosity}, \textit{use of markdown}).

\paragraph{Automated Attribute Extraction.} We employ an LLM, prompted with $Q$ and example responses, to propose a set of candidate causal attributes relevant to evaluating answers for $Q$. The prompt (see Appendix [Reference]) encourages the identification of key quality dimensions. Although the prompt may also produce importance scores for analysis, the primary output used in subsequent steps is the set of attributes $C$ and potential spurious attributes $SP$.

\paragraph{Refinement and Verification.} The LLM-generated attribute lists are reviewed for coherence and consistency. Semantically overlapping attributes may be merged, and automated checks can be applied to ensure the identified attributes align with the intended causal/spurious distinction.

\subsection{Step 2: Generating Counterfactual Augmented Data}
\label{subsec:counterfactual_generation}

Using the identified attributes, we generate synthetic data pairs designed to isolate the influence of $C$ and neutralize the influence of $SP$. This involves creating variations of existing answers $A$ (e.g., $y_w$ or $y_l$ from $\mathcal{D}_{pref}$).

\paragraph{Causal Augmentation.} To teach the model sensitivity to $C$, we generate pairs $(A, A')$ intended to differ primarily along a single causal attribute $C_j$. This is done through \emph{upgradation} (improving $A$ along $C_j$ to get $A'$) or \emph{degradation} (worsening $A$ along $C_j$ to get $A'$). For instance, given a factually correct answer $A$, we might generate a degraded version $A'$ containing a factual error but preserving style and length. The pair $(Q, A, A')$ would be labeled $A \succ A'$. Conversely, upgrading a poor answer $A$ to $A'$ yields a label $A' \succ A$. We use LLM prompts (Appendix [Reference]) that specify the target attribute $C_j$ and instruct the LLM to make "significant but isolated" modifications, aiming to keep other attributes $C_{k \neq j}$ and $SP$ constant.

\paragraph{Neutral Augmentation.} To teach the model invariance to $SP$, we generate pairs $(A_1, A_2)$ that ideally share the same causal attributes $C$ but differ in spurious attributes $SP$. These pairs are assigned a "tie" label ($y = \text{tie}$), helping the model learn to assign \emph{equal} reward when only spurious features differ. Our primary technique is \emph{causally-aligned reconstruction}. We first use an LLM to analyze the differences in causal attributes between two answers $A_1$ and $A_2$ (Appendix [Reference]). Then, we prompt the LLM (Appendix [Reference]) to rewrite $A_2$ to match the causal profile of $A_1$ while retaining the original style and spurious features of $A_2$ as much as possible. Let this reconstructed answer be $A'_{2 \to 1}$. The pair $(Q, A_1, A'_{2 \to 1})$ is labeled as $y = \text{tie}$. Symmetrically generating $A'_{1 \to 2}$ yields another tie pair $(Q, A_2, A'_{1 \to 2})$.

\subsection{Step 3: Filtering Augmented Data}
\label{subsec:filtering_revised}

The generation process in Step 2 can yield imperfect or uninformative examples. We apply filtering to refine the augmented dataset $\mathcal{D}_{aug}$ before training.

\paragraph{Model-based Confidence Filtering.} We prioritize augmentations that represent challenging or incorrectly assessed cases for a baseline model. Using a pre-trained baseline reward model, $\hat{R}_{base}$, we compute its prediction for each augmented pair. Let $p = P_{base}(B \succ A)$ for a pair $(A, B)$.
\begin{itemize}[itemsep=0pt,left=2pt]
    \item If the pair was generated with label $B \succ A$ (causal upgrade/degradation), we retain it only if the baseline model is not confident in the correct label, i.e., $|p - 1.0| > \tau$.
    \item If the pair was generated as a neutral tie ($y=\text{tie}$), we retain it only if the baseline model incorrectly assigns a strong preference, i.e., $|p - 0.5| > \tau$.
\end{itemize}
We use a threshold $\tau=0.2$, empirically chosen for consistency with related work \cite{liu2024rrm} and to focus training on pairs where the augmentation provides the most learning signal relative to the baseline.

\paragraph{Quality Verification.} We use further model based verification steps using automated scoring (e.g., fluency) to verify the validity of the generated pairs and their labels.

The result is the filtered augmented dataset, $\mathcal{D}_{aug\_filtered}$.

\subsection{Step 4: Training the Robust Reward Model}
\label{subsec:training_revised}

The final robust reward model $\hat{R}_\phi$ is trained on the combined dataset $\mathcal{D} = \mathcal{D}_{pref} \cup \mathcal{D}_{aug\_filtered}$. We minimize a composite loss function based on the Bradley-Terry framework that handles both standard preference pairs and the neutral tie pairs:
\begin{align}
\mathcal{L}(\phi) = &- \sum_{(Q, y_w, y_l) \in \mathcal{D}_{pref} \cup \mathcal{D}_{causal}} \log \sigmoid(\hat{R}_\phi(Q, y_w) - \hat{R}_\phi(Q, y_l)) \nonumber \\
&- \lambda \sum_{(Q, A_1, A_2, y=\text{tie})\in \mathcal{D}_{neutral}} [ \log \sigmoid(\Delta_{12}) + \log \sigmoid(-\Delta_{12}) ]
\label{eq:combined_loss_methodology_final_revised}
\end{align}
where $\Delta_{12} = \hat{R}_\phi(Q, A_1) - \hat{R}_\phi(Q, A_2)$. The first term is the standard negative log-likelihood loss. The second term, weighted by hyperparameter $\lambda \ge 0$, applies to the neutral pairs. This term encourages $\Delta_{12} \approx 0$ (equivalent to pushing $\sigma(\Delta_{12}) \to 0.5$), penalizing the model for assigning different scores to answers deemed causally equivalent. We tune $\lambda$ on a validation set (see Section \ref{sec:experiments}) to balance spurious invariance with causal sensitivity.

By optimizing $\mathcal{L}(\phi)$, the model internalizes the distinctions enforced by the augmentations. Creating pairs that vary $C$ while holding $SP$ constant (causal augmentation) and pairs that vary $SP$ while holding $C$ constant (neutral augmentation) helps break the spurious correlation path $(A \to SP \to \hat{y})$ present in naive training, guiding $\hat{R}_\phi$ to align more closely with the true causal path $(A \to C \to R)$.



==> archived/am_20250510.tex <==
\section{Methodology: Training a Robust Reward Model}
\label{sec:methodology}

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{images/DataAugmentationPipeline_new.pdf} % Assuming this path is correct
\caption{The \carma{} data augmentation pipeline. Original preference data ($\mathcal{D}_{\mathrm{pref}}$) is used as a basis to generate: (1) \textit{Causal Augmentations} ($\mathcal{D}_{\mathrm{causal}}$) by performing \textbf{Attribute Upgradation and Degradation} on specific attributes to enforce sensitivity to genuine quality drivers, and (2) \textit{Neutral Augmentations} ($\mathcal{D}_{\mathrm{neutral}}$) via Causally-Aligned Reconstructions and Irrelevant Pair Comparisons (with tie-labels) to teach spurious feature invariance. After optional filtering, the reward model is trained on the combined original and augmented dataset.}
\label{fig:data_augmentation_pipeline}
\end{figure}

The \carma{} framework employs a causally-motivated data augmentation strategy to train robust reward models. The process involves two main phases: generating attribute-aware counterfactual data based on the causal model (Section \ref{sec:preliminaries}), and then training the reward model using a specialized loss function on the combined original and augmented data, as illustrated in Figure \ref{fig:data_augmentation_pipeline}.

\subsection{Attribute-Aware Counterfactual Data Generation}
\label{subsec:data_generation_phase}

This phase prepares the augmented dataset $\mathcal{D}_{\mathrm{aug}} = \mathcal{D}_{\mathrm{causal}} \cup \mathcal{D}_{\mathrm{neutral}}$ required for robust training, involving three conceptual steps:

\paragraph{Step 1: Attribute Identification.}
As a prerequisite, we identify the Principal Causal Components $\mathrm{C} = (\mathrm{C}_1, \dots, \mathrm{C}_\ell)$ relevant to the task, leveraging the causal framework from Section \ref{subsec:causal_graph}. This typically involves LLM prompting and refinement (Details in Appendix~\ref{subsec:attribute_identification_appendix}).

\paragraph{Step 2: Counterfactual Generation.}
Using the identified attributes $\mathrm{C}$, we generate synthetic data pairs via LLM-approximated counterfactuals, as defined in Section \ref{subsec:approximating_counterfactuals}. Following the strategies summarized in Table \ref{tab:augmentation_summary} and detailed conceptually in Section \ref{subsec:data_augmentation}, we create:
\begin{itemize}[itemsep=0pt, left=10pt]
    \item \textit{Causal Augmentation Pairs} ($\mathcal{D}_{\mathrm{causal}}$): Examples enforcing sensitivity to individual causal attributes $\mathrm{C}_j$ via \textbf{Attribute Upgradation} and \textbf{Degradation}, with  standard preference labels ($\succ$).
    \item \textit{Neutral Augmentation Pairs} ($\mathcal{D}_{\mathrm{neutral}}$): Examples enforcing invariance to spurious attributes $\mathrm{SP}$ while holding causal content $\mathrm{C}$ constant or ensuring $\mathrm{C}$ is irrelevant. These are generated via \textbf{Causally-Aligned Reconstruction} and \textbf{Irrelevant Pair Comparison} (using query modification). These receive tie labels ($\approx$).
\end{itemize}
The specific LLM prompts driving this generation are provided in Appendix~\ref{sec:prompt_templates}. This step yields the raw augmented dataset $\mathcal{D}_{\mathrm{aug}}$.

\paragraph{Step 3: Data Filtering.}
To improve training efficiency, the raw $\mathcal{D}_{\mathrm{aug}}$ can be filtered into $\mathcal{D}_{\mathrm{aug\_filtered}}$. This often involves using a baseline model $\hat{\mathrm{R}}_{\mathrm{base}}$ (trained only on $\mathcal{D}_{\mathrm{pref}}$) to select only those augmented pairs where the baseline is uncertain or incorrect, thus focusing training on the most informative examples. Details on the filtering strategy and thresholds are provided in Section \ref{sec:experiments} and Appendix \ref{subsec:filtering_appendix}.

This data generation phase outputs the datasets $\mathcal{D}_{\mathrm{pref}}$ (original preferences) and $\mathcal{D}_{\mathrm{aug\_filtered}}$, which serve as input to the model training phase.

\subsection{Robust Reward Model Training}
\label{subsec:training_phase}

Given the original data $\mathcal{D}_{\mathrm{pref}}$ and the filtered augmented data $\mathcal{D}_{\mathrm{aug\_filtered}}$, the final \carma{} reward model $\hat{\mathrm{R}}_\theta$ is trained by minimizing a composite loss function $\mathcal{L}(\theta)$ over the combined dataset $\mathcal{D} = \mathcal{D}_{\mathrm{pref}} \cup \mathcal{D}_{\mathrm{aug\_filtered}}$:
\begin{align}
\mathcal{L}(\theta) = &- \underbrace{\sum_{(\mathrm{Q}, \mathrm{y}_w, \mathrm{y}_l) \in \mathcal{D}_{\mathrm{pref}} \cup \mathcal{D}_{\mathrm{causal}}} \log \sigmoid(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{y}_w) - \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{y}_l))}_{\text{Preference Loss (Causal Sensitivity)}} \nonumber \\
&- \lambda \underbrace{\sum_{(\mathrm{Q}, \mathrm{A}_1, \mathrm{A}_2, y=\text{tie})\in \mathcal{D}_{\mathrm{neutral}}} \left( -\frac{1}{2} \left[ \log \sigmoid(\Delta_{12}) + \log \sigmoid(-\Delta_{12}) \right] \right)}_{\text{Neutral Tie Loss (Spurious Invariance)}}
\label{eq:combined_loss_methodology}
\end{align}
where $\Delta_{12} = \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2)$.
The first component is the standard Bradley-Terry negative log-likelihood loss, applied to $\mathcal{D}_{\mathrm{pref}}$ and the Causal Augmentation pairs $\mathcal{D}_{\mathrm{causal}}$. It ensures the model learns to prefer responses with higher causal quality, aligning with the ground truth $\mathrm{R}^*$ and the specific attribute manipulations.

The second component specifically targets the neutral pairs $\mathcal{D}_{\mathrm{neutral}}$ to enforce invariance. The tie loss term encourages the model score difference $\Delta_{12}$ to approach zero for pairs that differ only spuriously (or are both equally irrelevant), effectively penalizing reliance on $\mathrm{SP}(\mathrm{A})$ when $\mathrm{C}(\mathrm{A})$ is constant or irrelevant. The hyperparameter $\lambda \ge 0$ balances these two objectives, controlling the strength of the enforced spurious invariance relative to fitting preferences; its value is determined experimentally (Section \ref{sec:experiments}).

Optimizing this composite loss $\mathcal{L}(\theta)$ trains $\hat{\mathrm{R}}_\theta$ to be simultaneously sensitive to the identified causal attributes $\mathrm{C}$ and robustly invariant to the variations in spurious attributes $\mathrm{SP}$ captured by the neutral augmentations. We will show experimental verification of such mitigation of reward hacking through downstream experiments on RewardBench and Re-word Bench \citep{lambert2024rewardbench,wu2025rewordbench}. Furthermore, we also show improved generation performance when we use this reward model for best-of-n sampling, as well as policy optimization in the DPO/MPO training loop.

==> archived/contrib_20250510.tex <==
\subsection{Our Contributions}
\label{subsec:our_contributions}

In this work, we address the persistent challenge of \emph{reward hacking} in large language model alignment by proposing \textbf{\carma{} (Causal Augmentation to disentangle Reward Modeling Attributes)}. Our main contributions are as follows:

\begin{itemize}[left=2pt,itemsep=0pt]
    \item \textbf{A Principled Causal Framework for Reward Modeling.}
    We propose a principled causal framework (Section~\ref{sec:preliminaries}, Figure~\ref{fig:causal_graph}) that explicitly models answer generation, distinguishing fundamental \emph{causal} drivers of quality (e.g., factual correctness, logical coherence) from \emph{spurious} correlates (e.g., stylistic choices, formatting). This framework underpins \carma{}'s design to train reward models that are sensitive to genuine quality and robust to superficial cues.

    \item \textbf{Targeted Data Augmentation via Counterfactuals.}
    Leveraging our causal model, we develop targeted data augmentation strategies (Section~\ref{sec:methodology}) using LLM-generated counterfactuals. These comprise: (1) \emph{Causal Augmentations}, creating minimal pairs that isolate changes in specific causal attributes to instill sensitivity to true quality differences, and (2) \emph{Neutral Augmentations}, varying spurious attributes while preserving causal content and using tie-labels to enforce invariance. We detail a systematic generation and filtering process for these informative examples.

    \item \textbf{Theoretical Analysis of Reward Hacking Mitigation.}
    We present a formal theoretical analysis (Section~\ref{sec:theory}) demonstrating that training with \carma{}'s augmentation scheme guides the reward model towards causal faithfulness. Under defined data coverage and optimization assumptions, our analysis shows this process discourages reliance on spurious attributes, and proves that an RM optimally fitting the augmented data would be robust against reward hacking via superficial manipulations.

    \item \textbf{State-of-the-Art Empirical Performance on Reward Benchmarks.}
    We conduct comprehensive experiments on \textbf{RewardBench} (Section~\ref{sec:experiments}), demonstrating that \carma{} significantly outperforms both standard reward models and the strong RRM baseline \citep{liu2024rrm}. Our approach yields substantial accuracy improvements across diverse categories, notably increasing Safety accuracy by up to \textbf{13.4\%} and Reasoning accuracy by up to \textbf{5.4\%} points (Tables~\ref{tab:results_pairpm_rewardbench}, \ref{tab:results_bt_rewardbench}).

    \item \textbf{Downstream Alignment Benefits.}
    Beyond static preference accuracy, we show that selecting Best of N (BoN)  responses from the policy model based on our reward model gives performance improvement of up to 10\% on AlpacaEval. Furthermore, policies trained via direct preference optimization (DPO) using \carma{}-based reward models exhibit less reward hacking tendencies and more robust performance, indicating the practical alignment advantages of our approach.

\end{itemize}


==> archived/es_20250510.tex <==
\subsection{Experimental Settings}
\label{subsec:experimental_settings}

\paragraph{Datasets.}
Our primary source of human preference data ($\mathcal{D}_{pref}$) is the Ultrafeedback dataset \cite{cui2023ultrafeedback}, containing approximately 60k preference pairs across diverse domains. For checking robustness to training data, we provide ablations with training data generated from the UltraInteract dataset \cite{yuan2024advancing} as well. The data augmentation process, following Section \ref{sec:methodology}, employs Gemini 2.0 Flash to identify $\ell=5$ causal attributes and subsequently generate causal upgrade/degradation pairs targeting these attributes, alongside neutral pairs using our reconstruction method. This augmented data $\mathcal{D}_{aug}$ is then filtered using a model-based confidence filter with threshold $\tau=0.2$, applied to a baseline RM trained solely on $\mathcal{D}_{pref}$. The final training set $\mathcal{D} = \mathcal{D}_{pref} \cup \mathcal{D}_{aug\_filtered}$ typically contains 3-3.5 times the number of examples in $\mathcal{D}_{pref}$. This is obtained as follows. First, we vary the positives and negatives with 5 counterfactuals each (corresponding to 5 causal attributes). This leads us to 10 times the original dataset size. Then we augment the neutrals to include positive and negative neutrals corresponding to 2 times the original size. Finally we verify and filter the data leaving us with 3-3.5 times the original dataset size.

\paragraph{Models.}
We instantiate our reward models using state-of-the-art transformer architectures, specifically Qwen2.5 7b \cite{yang2024qwen2} and Gemma2 9b \cite{team2024gemma}. Our primary architecture is the pairwise preference model, where input follows the format `Q, A, B`, and the model predicts a preference token ('A' or 'B'), which is trained using a cross entropy loss. We call this variant as $\carma\text{-PairPM}$. We propose another variant called $\carma \text{-BT}$

For downstream alignment, we fine-tune the corresponding base LLMs (Qwen2.5 7b, Gemma2 9b) using Direct Preference Optimization (DPO) \cite{rafailov2024direct} and Multi Preference Optimization (MPO) \cite{gupta2024swepo}.

\paragraph{Baselines and Ablations.}
We compare our full \carma{} approach against several alternatives. The primary baseline is a \textbf{Base RM} trained solely on $\mathcal{D}_{pref}$. We also compare against the \textbf{RRM Baseline} \cite{liu2024rrm}, which employs a different augmentation strategy involving non-contextual examples. 
Concretely, the \textsc{Rrm} Baseline augments using non-contextual examples, as well as examples from responses from different queries --- which are not specifically aligned with causal and spurious attributes. 
Ablations include training \carma{} with only causal augmentations (\textbf{\carma-Causal}, equivalent to $\lambda=0$), only neutral augmentations (\textbf{\carma-Neutral}), and exploring various weights for the neutral loss term (\textbf{\carma{} with varying $\lambda \in \{0.1, 0.5, 1.0, 2.0, 5.0\}$}). Additionally, we may compare our neutral generation method against alternatives like paraphrasing or temperature sampling.

\paragraph{Training Details.}
All models are trained in PyTorch using Hugging Face Transformers library. Reward models are trained for 1 epoch with the AdamW optimizer \cite{loshchilov2017decoupled}, a learning rate of $1e-6$, and a global batch size of $256$, employing a cosine learning rate schedule. DPO policy training proceeds for 1 epoch using AdamW, with a learning rate of $1e-6$, batch size $256$, and DPO $\beta = 0.01$.

\paragraph{Evaluation.}
Reward model quality is assessed using accuracy on the \textbf{RewardBench} benchmark \cite{lambert2024rewardbench}, with performance broken down by category (Chat, Chat-Hard, Safety, Reasoning). Robustness may be further evaluated using \textbf{Re-word Bench} \cite{wu2025rewordbench}. Policy performance is measured using standard alignment benchmarks: \textbf{MT-Bench} \cite{zheng2023judging} for multi-turn conversational ability (judged by GPT-4), and \textbf{AlpacaEval 2} \cite{alpaca_eval} for single-turn instruction following, reporting both standard and length-controlled (LC) win rates against reference models. We also analyze the \textbf{average response length} of the policies to evaluate verbosity bias and conduct \textbf{qualitative analysis} of generated responses to identify variations and failure models.

==> archived/expts_20250516.tex <==
\section{Experiments}
\label{sec:experiments}

\begin{table}[h]
    \centering
    \caption{Performance Comparison of Pairwise Preference Model and Bradley-Terry Reward Model on RewardBench trained using various base models}
    \label{tab:performance_bt_pairpm_rewardbench_extended_final} % Updated label
    % Adjusts width to text width, height is scaled proportionally
    \resizebox{\linewidth}{!}{%
    \renewcommand{\arraystretch}{1.3}% Increase row spacing for this table
    \begin{tabular}{@{}llHccccHccccc@{}}
        \toprule
        & \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{PairPM}} & \multicolumn{5}{c}{\textbf{BT}} \\
        \cmidrule(lr){3-7} \cmidrule(lr){8-12}
        & & \textbf{Average} & \textbf{Chat} & \textbf{Chat-Hard} & \textbf{Safety} & \textbf{Reasoning} & \textbf{Average} & \textbf{Chat} & \textbf{Chat-Hard} & \textbf{Safety} & \textbf{Reasoning} \\
        \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\small\gemmait{9}}}
        & Vanilla RM & 80.61 & \textbf{98.18} & 63.38 & 76.08 & 84.80 & 79.23 & \textbf{97.49} & 59.49 & 68.25 & 91.71 \\
        & RRM        & 82.53 & 96.93 & 72.04 & 73.78 & 87.36 & 83.22 & 97.49 & \textbf{68.53} & 73.18 & 93.68 \\
        & \textbf{\carma{}} & \textbf{87.93} & 97.49 & \textbf{72.70} & \textbf{86.96} & \textbf{94.55} & \textbf{85.33} & 96.09 & 66.12 & \textbf{82.84} & \textbf{96.27} \\
        \cmidrule(lr){2-12} 
        & $\Delta_{\text{\carma{} - RRM}}$ &
        \changeUp{+5.40} & 
        \changeUp{+0.56} &  
        \changeUp{+0.66} & 
        \changeUp{+13.18} & 
        \changeUp{+7.19} & 
        \changeUp{+2.11} &
        \changeDown{-1.40} & 
        \changeDown{-2.41} &
        \changeUp{+9.66} & 
        \changeUp{+2.59} \\ 
        \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\small\qwen{}}}
        & Vanilla RM & 78.18 & \textbf{97.21} & 52.85 & 73.99 & 88.68 & 72.73 & 97.21 & 46.27 & 68.04 & 79.39 \\
        & RRM        & 82.04 & 97.21 & \textbf{64.80} & 75.27 & 90.86 & 78.20 & \textbf{98.04} & \textbf{59.65} & 72.43 & 82.66 \\
        & \textbf{\carma{}} & \textbf{83.15} & 96.37 & 61.73 & \textbf{82.23} & \textbf{92.26} & \textbf{80.81} & 96.93 & 58.66 & \textbf{78.92} & \textbf{88.71} \\
        \cmidrule(lr){2-12} 
        & $\Delta_{\text{\carma{} - RRM}}$ &
        \changeUp{+1.11} &
        \changeDown{-0.84} &
        \changeDown{-3.07} &
        \changeUp{+6.96} &
        \changeUp{+1.40} &
        \changeUp{+2.61} &
        \changeDown{-1.11} &
        \changeDown{-0.99} & 
        \changeUp{+6.49} &
        \changeUp{+6.05} \\
        \midrule % Added midrule for separation
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\small\gemma{2}}} % New model block
        & Vanilla RM & 53.75 & 92.88 & 33.33 & 42.03 & 46.74 & 65.52 & 94.27 & 38.27 & 50.20 & 79.34 \\
        & RRM        & 66.23 & \textbf{94.13} & 43.75 & 47.64 & 79.38 & 66.95 & \textbf{94.97} & 49.34 & 50.07 & 73.42 \\
        & \textbf{\carma{}} & \textbf{70.69} & 92.18 & \textbf{50.00} & \textbf{55.14} & \textbf{85.42} & \textbf{72.45} & 92.74 & \textbf{53.62} & \textbf{60.00} & \textbf{83.45} \\
        \cmidrule(lr){2-12} 
        & $\Delta_{\text{\carma{} - RRM}}$ &
        \changeUp{+4.46} &
        \changeDown{-1.95} &  
        \changeUp{+6.25} & 
        \changeUp{+7.50} & 
        \changeUp{+6.04} & 
        \changeUp{+5.50} &
        \changeDown{-2.23} & 
        \changeUp{+4.28} &
        \changeUp{+9.93} & 
        \changeUp{+10.03} \\ 
        \bottomrule
    \end{tabular}%
    }
\end{table}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=1.0\columnwidth]{images/reword_absolute_robustness_gemma9b_pairpm_sorted.pdf}
  \caption{Absolute robustness comparison of RM, RRM and \carma{} on reWordBench.
  % in the PairPM setup, for reward models built over \texttt{Gemma-2-9B-IT}.
  }
  \label{fig:reword_absolute_robustness_gemma9b_pairpm}
  
\end{figure}

In this section we evaluate \carma{}'s reduced reliance on spurious attributes and closer alignment of the learned reward model with true causal attributes. We empirically evaluate improvements obtained by \carma{} in standard preference classification settings, tests designed to evaluate reward model robustness and how gains in robustness translate to better language model alignment.

Our experiments are designed to addreess the following research questions:


% We empirically evaluate CARMA's causal data augmentation strategy (Section \ref{sec:methodology}). Our experiments investigate if CARMA improves reward model (RM) performance, enhances robustness against spurious attributes, and leads to better downstream policy alignment compared to baselines.

% \label{list:research_questions}
% \begin{itemize}[left=18pt,itemsep=2pt]
%     \item[\textbf{RQ1}] \textbf{Effectiveness of Augmentation Components} How do the causal and neutral augmentation components individually contribute to the performance and robustness of \carma{} Specifically, does neutral augmentation enhance SP-invariance, and does causal augmentation maintain C-sensitivity?
%     \item[\textbf{RQ2}] \textbf{Robustness} Does \carma{} improve the robustness of the learned reward model against known spurious correlations (e.g., length, formatting bias) compared to a standard RM trained only on $\mathcal{D}_{pref}$ and the RRM baseline?
%     \item[\textbf{RQ3}] \textbf{Downstream Policy Alignment} Do policies aligned using $\hat{R}_{\carma}$ (via DPO) achieve better performance on standard alignment benchmarks (e.g., MT-Bench, AlpacaEval-2) and exhibit less reward hacking behavior compared to policies aligned using baseline RMs?
%     \item[\textbf{RQ4}] \textbf{Assessing Performance of Neutrals} 
%     How do different type of Neutral generations, viz. paraphrasing, rewrites, question-independence, affect downstream performance for reward modeling?
% \end{itemize}

\label{list:research_questions}
\begin{itemize}[left=18pt,itemsep=2pt, topsep=0pt, parsep=2pt]
    % \item[\textbf{RQ1:}] \textbf{RM Performance and Robustness:} How does \carma{} perform on standard preference benchmark \textbf{RewardBench} and how robust is it against \textit{ranking-preserving} adversarial transformations proposed in \textbf{reWordBench} designed to expose reliance on spurious correlations compared to baselines?
    \item[\textbf{RQ1:}] \textbf{RM Performance and Robustness:} How does \carma{} perform on standard preference prediction tasks and how robust is it against spurious correlations compared to a standard RM and strong baselines trained on $\mathcal{D}_{pref}$ (Table \ref{tab:performance_bt_pairpm_rewardbench_extended_final}, Figure \ref{fig:reword_absolute_robustness_gemma9b_pairpm})?    

    \item[\textbf{RQ2:}] \textbf{Policy Alignment:} Does the robustness achieved by \carma{} lead to more favorable results in a Best-of-N policy alignment setup, compared to strong baselines (Figure \ref{fig:bon_asr_reduction_gsm8k_gemma9b})? \todohs{Pragya to add BoN rewordbench fig reference here} 
    
    % Whaten policies are aligned using \carma{} RMs via Best-of-N response selection, do they achieve superior performance and, crucially, exhibit less reward hacking across a diverse suite of benchmarks — spanning general helpfulness (\textbf{AlpacaEval 2}), mathematical reasoning (\textbf{GSM8K}) and robustness to adversarial prompts (\textbf{WildGuardTest}) as compared to policies aligned with baseline RMs?
    % {\color{orange}: PS: Update this after we have all the BoN numbers}
    \item[\textbf{RQ3:}] \textbf{Neutral Augmentations:} How effective are the different neutrals augmentation strategies in enforcing \textit{invariance} to unknown spurious correlates (Figures \ref{fig:rewardbench_subsets_neutral_ablations}, \ref{fig:rewordbench-avg_neutral_ablations})?
\end{itemize}


\input{includes/experimental_settings}
\input{includes/experimental_results}



==> archived/extended_related_works_20250501.tex <==
\section{Related Works}
\label{sec:related_works} % Changed from extended_related_works for standard naming

Our work on \carma{}, a framework for causally robust reward modeling, intersects with and builds upon several key areas of research: the alignment of Large Language Models (LLMs) via human feedback, techniques for reward model training, the persistent challenge of reward hacking, the application of causal inference principles to machine learning, and data augmentation strategies for enhancing model robustness.

\paragraph{LLM Alignment and RLHF.}
The dominant paradigm for steering LLM behavior towards desired attributes like helpfulness, honesty, and harmlessness is Reinforcement Learning from Human Feedback (RLHF) \citep{christiano2017deep, stiennon2020learning, ouyang2022training, bai2022training, askell2021general}. The standard RLHF process involves training a reward model (RM) on human preferences (typically pairwise comparisons) and subsequently using this RM as a reward signal to fine-tune the LLM policy via RL algorithms such as PPO \citep{schulman2017proximal}. The quality, calibration, and robustness of the RM are paramount, as flaws in the RM directly impact the alignment outcome \citep{casper2023open}. While alternative alignment algorithms like Direct Preference Optimization (DPO) \citep{rafailov2024direct} and its extensions (e.g., IPO \citep{azar2024general}, KTO \citep{ethayarajh2024kto}, ORPO \citep{hong2024orpo}, SimPO \citep{meng2024simpo}) bypass explicit RM training by directly optimizing the policy on preference data, they still implicitly rely on the preference information learnable from the data, making the problem of distinguishing true quality from spurious correlates equally relevant. Community efforts like OpenAssistant have also contributed significantly by crowdsourcing preference data \citep{köpf2023openassistant}.

\paragraph{Reward Modeling Techniques.}
Learning accurate reward models from preference data remains a central challenge. Methodologies primarily include Bradley-Terry style pointwise models that learn a scalar score $r(x, y)$ \citep{bradley1952rank, ouyang2022training, bai2022training}, and pairwise ranking models that directly predict preference probabilities, often implemented within the LLM architecture itself (PairPM) \citep{rafailov2024direct, liu2025pairwise, qin2023large}. Other approaches explore Q-function based rewards \citep{li2024process} or process supervision \citep{khalifa2025process}. Significant effort focuses on improving specific RM properties like calibration \citep{zhu2025charm, zhao2023slic}, training efficiency \citep{tunstall2023zephyr, wu2023zephyr}, uncertainty quantification \citep{lou2024uncertainty}, interpretability through multi-aspect rewards \citep{wang2024interpretable, yang2024rewards, xu2024multiaspect}, and scalability via reasoning or chain-of-thought mechanisms \citep{zhao2025genprm}. Our work complements these efforts by focusing specifically on enhancing the causal \textbf{robustness} of the learned reward function $\hat{R}$ against spurious attributes.

\paragraph{Reward Hacking and Spurious Correlations.}
Learned reward models are notoriously susceptible to \textit{reward hacking} or \textit{over-optimization} \citep{gao2023scaling, skalse2022defining, pan2022effectsrewardmisspecificationmapping}. Because RMs are trained on finite, potentially biased data, they often learn to associate high rewards with superficial or \textit{spurious} features that are merely correlated with desirable responses in the training set but do not reflect true quality. Common examples include excessive length or verbosity \citep{singhal2023long, liu2023llm}, specific formatting patterns like lists or markdown \citep{zhang2024lists, zhang2024emojis}, adherence to stylistic conventions like politeness, or even sycophantic agreement with user views \citep{denison2024sycophancy, dennison2024measuring}. Policies optimized against such RMs learn to exploit these spurious cues, leading to outputs that maximize the predicted reward but fail to align with genuine human preferences or task goals \citep{shen2023trickle}.

\paragraph{Approaches to Mitigating Reward Hacking.}
Various strategies have been proposed to address reward hacking. Model-centric approaches include using ensembles of RMs to average out idiosyncratic biases \citep{coste2023reward, eisenstein2023helping, rame2024warm}, incorporating explicit calibration methods \citep{zhao2023slic}, or designing architectures that factorize reward components, such as ODIN's disentanglement of quality and length \citep{chen2024odin, chen2023odin}. Policy-optimization techniques might involve adding explicit penalties for spurious features (e.g., length penalties \citep{park2024disentangling}) or using specific regularization methods during fine-tuning \citep{radford2019language}. Data-centric approaches aim to improve the training data or process itself. Examples include iterative re-labeling or refinement (e.g., Constitutional AI \citep{bai2022constitutional}), performing consistency checks across related prompts \citep{shen2023trickle}, adversarial red-teaming \citep{ganguli2022red}, and augmenting the dataset with synthetic examples designed to improve robustness \citep{pace2024west, shen2024boosting, liu2024rmboost}. Our work, \carma{}, falls firmly in this data-centric category. It is closely related to RRM \citep{liu2024rrm}, which also uses data augmentation (non-contextual and query-independent pairs) for robustness. However, \carma{} is distinct in its use of an explicit causal framework and its generation of targeted, attribute-specific counterfactuals to disentangle causal from spurious factors.

\paragraph{Causal Inference in Machine Learning.}
Causal inference provides formal tools, such as Structural Causal Models (SCMs) and Directed Acyclic Graphs (DAGs) \citep{pearl2009causality, pearl2000causality, peters2017elements}, for reasoning about cause-effect relationships, confounding, and counterfactuals. Applying causal principles in machine learning aims to build models that are more robust, fair, and interpretable by focusing on underlying causal mechanisms rather than potentially brittle statistical correlations \citep{scholkopf2021toward, scholkopf2022causality}. Techniques like Invariant Risk Minimization (IRM) seek models that perform well across different environments by relying on invariant (presumably causal) predictors \citep{arjovsky2019invariant, arjovsky2020invariant, ahuja2021irmv1}. Our work adopts this causal perspective, framing spurious attributes as non-causal factors whose influence on the learned reward model should be minimized.

\paragraph{Causality in LLMs and NLP.}
The intersection of causality and LLMs is rapidly evolving. Research includes probing the innate causal reasoning abilities of LLMs \citep{kiciman2023causal, chi2024unveiling}, leveraging LLMs as tools for automating parts of the causal discovery or analysis pipeline \citep{long2023causal, tu2023causal}, and applying causal methods to enhance NLP tasks. For instance, counterfactual reasoning and data augmentation have been used to improve robustness against biases in text classification \citep{kaushik2019learning, kaushik2020cda, qian2023counterfactual, feder2021causalm} and assess fairness \citep{feder2022causal}. In reward modeling, CARMO \citep{gupta2025carmodynamiccriteriageneration, gupta2025carmo} uses LLMs to dynamically generate evaluation criteria, linking to attribute-based assessment. \carma{} uniquely employs a predefined causal graph to structure the generation of counterfactual data specifically for training a robust RM, using LLMs as the generation engine.

\paragraph{Data Augmentation for Robustness.}
Data augmentation is a cornerstone technique for improving model generalization. Beyond traditional NLP methods like synonym replacement or back-translation \citep{wu2025rewordbench}, more recent approaches leverage LLMs for sophisticated augmentations, including paraphrasing, style transfer, generating adversarial examples \citep{qiang2024prompt}, or creating counterfactuals \citep{mishra2024llm, feder2021causalm, yang2021causalcnn}. Methods based on sampling, like Gumbel temperature sampling, have also been explored for counterfactual generation \citep{ravfogel2025gumbelcounterfactualgenerationlanguage}. Contrastive methods, such as contrastive instruction tuning \citep{shen2023contrastive}, perturb inputs to enforce invariance. Counterfactual data augmentation, particularly generating minimally different pairs to isolate specific features \citep{kaushik2019learning}, is highly relevant. Our work operationalizes this concept within a causal framework, generating targeted "causal" and "neutral" pairs to enforce specific invariance and sensitivity properties in the RM. Curriculum-based strategies \citep{gou2023curriculum} could potentially integrate with our attribute-wise augmentation schedule.

\paragraph{Positioning of \carma.}
\carma{} integrates insights from causal inference and data augmentation to address the critical problem of reward hacking in LLM alignment. While related works like RRM \citep{liu2024rrm} use data augmentation for robustness and CARMO \citep{gupta2025carmodynamiccriteriageneration} uses LLMs for criteria generation, \carma{} is distinguished by its explicit grounding in a causal graph model of answer attributes. It systematically generates attribute-specific counterfactual and neutral examples via guided LLM prompting to directly train the RM to distinguish causal quality drivers ($C$) from spurious correlates ($SP$). This allows \carma{} to potentially handle a wider range of spurious attributes beyond commonly studied ones like length, aiming for a more principled and generalizable form of robustness. We provide the methodology and empirical validation (Section \ref{sec:experiments}) demonstrating that this causally-informed data augmentation leads to more robust reward models and better downstream policy alignment compared to standard baselines.

==> archived/intro_20250509.tex <==
\section{Introduction}
\label{sec:introduction}

Aligning Large Language Models (LLMs) with human preferences is paramount for their safe and effective deployment. Reinforcement Learning from Human Feedback (RLHF) methods relying on reward models (RMs) have emerged as the dominant paradigm for this task \citep{christiano2017deep, ouyang2022training, bai2022training,schulman2017proximal,shao2024deepseekmath}. 
% , typically relying on a reward model (RM) trained on human preference data, often pairwise comparisons \citep{bradley1952rank}. 
This learned RM serves as a proxy for human judgment, guiding policy optimization via algorithms like PPO \citep{schulman2017proximal} or through direct preference optimization methods like DPO \citep{rafailov2024direct}. The fidelity and robustness of the RM are critical, as flaws directly propagate to the aligned policy \citep{casper2023open}.

However, standard RM training faces a significant challenge --- \textit{reward hacking} \citep{gao2023scaling, skalse2022defining}. RMs often learn to assign high scores based on superficial or spurious attributes—such as response length \citep{singhal2023long}, specific formatting patterns \citep{zhang2024lists}, or stylistic quirks, mainly because these features are statistically correlated with preferred responses in the training dataset. This occurs because standard training objectives, like minimizing pairwise preference prediction error, do not explicitly require the RM to disentangle the true \textit{causal} drivers of response quality (e.g., factuality, relevance, coherence) from these spurious correlates. Consequently, RMs may become brittle, exhibiting poor generalization and enabling policies to maximize predicted reward via superficial manipulations rather than genuine quality improvements \citep{shen2023trickle, eisenstein2023helping}.

To address spurious correlations in reward modeling, recent works have explored several methods for robustness, sometimes drawing on causal concepts. The \rewordbench{} benchmark \citep{wu2025rewordbench} highlighted the brittleness of RMs to meaning-preserving input transformations and proposed regularizing RMs for consistency on paraphrased inputs as a mitigation strategy. \citet{liu2024rrm} introduced \rrm, employing data augmentation with non-contextual and query-independent response pairs to disrupt certain spurious associations learned from the context. Concurrently, attribute-based evaluation, such as dynamically generating criteria via LLMs as in \carmo{} \citep{gupta2025carmodynamiccriteriageneration}, aims to provide more grounded reward signals by focusing on specific quality dimensions.

However, these approaches exhibit certain limitations. Paraphrase regularization \citep{wu2025rewordbench} and MMD regularization for length bias and sycophantic bias \citep{wang2025beyond}, address only specific types of spurious variation; moreover, the complete set of spurious correlates may not be specifiable a priori. Furthermore, the method does not explicitly amplify the signal from underlying causal quality attributes.
% Similarly, other causal-inspired approaches like the MMD regularization method proposed by \citet{wang2025beyond} require explicit identification and pre-specification of spurious factors to enforce independence, which may not capture all relevant correlations or be feasible in complex scenarios.
Conversely, methods like RATE \citep{reber2024rate} emphasize causal estimation via ``rewrite of rewrites'', rather than directly training robust RMs through augmentation with causal and neutrality constraints.
% Conversely, methods like RATE \citep{reber2024rate}, while offering a sophisticated way to estimate causal effects by correcting for imperfect counterfactual generation using 'rewrites of rewrites', primarily focus on evaluation and causal estimation rather than directly providing a framework for training robust reward models via augmenting the learning process with both causal sensitivity and spurious invariance constraints.
\rrm's augmentation strategy, while improving general robustness, operates at a coarse level (swapping entire responses) and lacks fine-grained control to isolate the effects of specific causal or spurious attributes within a response. \carmo, focusing on criteria generation for evaluation, relies heavily on large LLMs at inference time, potentially incurring significant costs, and does not directly intervene on the RM's training data distribution using counterfactuals to enforce desired robustness properties like invariance. There remains a need for a method that systematically leverages a causal understanding of preference formation to train RMs that are directly sensitive to causal factors and robustly invariant to a wider range of spurious ones.


To address this gap, we propose \textbf{\carma{}} (Causal Attribute-aware Reward Modeling), a novel framework grounded in the explicit causal model of answer generation and evaluation introduced earlier (Section \ref{sec:preliminaries}, Figure \ref{fig:causal_graph}). The core idea of \carma{} is to directly teach the reward model to differentiate between genuine quality drivers and superficial cues by augmenting the standard preference dataset with targeted, LLM-generated counterfactual examples. This involves creating two key types of synthetic training pairs: (1) \textit{Causal Augmentation}, which generates minimally different responses that isolate changes along specific attributes identified as \textit{causal} (like factuality or relevance), thereby explicitly teaching the model sensitivity to genuine quality improvements or degradations. (2) \textit{Neutral Augmentation}, which produces pairs that vary primarily in \textit{spurious} ways (such as style or formatting) while preserving the core causal content, explicitly training the model for invariance to these superficial changes via tie-labels. By training on this enriched dataset using a modified preference loss (detailed in Section \ref{sec:methodology}), \carma{} learns a reward function that aligns more closely with the underlying causal factors of quality. %, leading to demonstrably improved robustness and better downstream policy alignment, as shown in our empirical evaluations.
Our empirical evaluations demonstrate that \carma{} leads to significantly improved robustness, boosting average accuracy on RewardBench by up to 4.5 percentage points over standard baselines, with significant gains in safety and reasoning capabilities.

The remainder of this paper details our causal framework (Section \ref{sec:preliminaries}), the \carma{} methodology (Section \ref{sec:methodology}), theoretical justifications (Section \ref{sec:theory}), and comprehensive experimental results (Section \ref{sec:experiments}) which address key \hyperref[list:research_questions]{research questions} towards robust reward modeling.

% To address this gap, we propose \textbf{\carma{}} (Causal Attribute-aware Reward Modeling), a novel framework grounded in an explicit causal model of answer generation and evaluation (Section \ref{sec:preliminaries}, Figure \ref{fig:causal_graph}). Our core idea is to directly train the RM to distinguish causal attributes ($C$) from spurious attributes ($SP$) by augmenting the standard preference dataset $\mathcal{D}_{pref}$ with targeted, LLM-generated counterfactual examples ($\mathcal{D}_{aug}$). Specifically, \carma{} employs two key augmentation types: (1) \textit{Causal Augmentation}, creating minimally different response pairs that isolate changes along specific causal attributes ($C_j$) to explicitly teach the RM sensitivity to factors like factuality or relevance, and (2) \textit{Neutral Augmentation}, generating pairs that differ primarily in spurious attributes ($SP$) but are equivalent in causal content ($C$) and thus labeled as ties, explicitly teaching the RM invariance to superficial variations like style or formatting. By training on the combined dataset using a modified pairwise loss (Section \ref{sec:methodology}), \carma{} learns a reward function that more closely reflects the ground-truth causal structure $R(Q, C)$, demonstrably improving robustness and downstream alignment performance as shown in our empirical evaluations.



==> archived/intro_20250510.tex <==
\section{Introduction}
\label{sec:introduction}

Aligning Large Language Models (LLMs) with human preferences is paramount for their safe and effective deployment. Reinforcement Learning from Human Feedback (RLHF) methods relying on reward models (RMs) have emerged as the dominant paradigm for this task \citep{christiano2017deep, ouyang2022training, bai2022training,schulman2017proximal,shao2024deepseekmath}. 
This learned RM serves as a proxy for human judgment, guiding policy optimization via algorithms like PPO \citep{schulman2017proximal} or through direct preference optimization methods like DPO \citep{rafailov2024direct}. The fidelity and robustness of the RM are critical, as flaws directly propagate to the aligned policy \citep{casper2023open}.

However, standard RM training faces a significant challenge --- \textit{reward hacking} \citep{gao2023scaling, skalse2022defining}. RMs often learn to assign high scores based on superficial or spurious attributes—such as response length \citep{singhal2023long}, specific formatting patterns \citep{zhang2024lists}, or stylistic quirks, mainly because these features are statistically correlated with preferred responses in the training dataset. This occurs because standard training objectives, like minimizing pairwise preference prediction error, do not explicitly require the RM to disentangle the true \textit{causal} drivers of response quality (e.g., factuality, relevance, coherence) from these spurious correlates. Consequently, RMs may become brittle, exhibiting poor generalization and enabling policies to maximize predicted reward via superficial manipulations rather than genuine quality improvements \citep{shen2023trickle, eisenstein2023helping}.

To address spurious correlations in reward modeling, recent works have explored several methods for robustness, sometimes drawing on causal concepts. The \rewordbench{} benchmark \citep{wu2025rewordbench} highlighted the brittleness of RMs to meaning-preserving input transformations and proposed regularizing RMs for consistency on paraphrased inputs as a mitigation strategy. \citet{liu2024rrm} introduced \rrm, employing data augmentation with non-contextual and query-independent response pairs to disrupt certain spurious associations learned from the context. Concurrently, attribute-based evaluation, such as dynamically generating criteria via LLMs as in \carmo{} \citep{gupta2025carmodynamiccriteriageneration}, aims to provide more grounded reward signals by focusing on specific quality dimensions.

However, these approaches exhibit certain limitations. Paraphrase regularization \citep{wu2025rewordbench} and MMD regularization for length bias and sycophantic bias \citep{wang2025beyond}, address only specific types of spurious variation; moreover, the complete set of spurious correlates may not be specifiable a priori. Furthermore, the method does not explicitly amplify the signal from underlying causal quality attributes.
Conversely, methods like RATE \citep{reber2024rate} emphasize causal estimation via ``rewrite of rewrites'', rather than directly training robust RMs through augmentation with causal and neutrality constraints.
\rrm's augmentation strategy, while improving general robustness, operates at a coarse level (swapping entire responses) and lacks fine-grained control to isolate the effects of specific causal or spurious attributes within a response. \carmo, focusing on criteria generation for evaluation, relies heavily on large LLMs at inference time, potentially incurring significant costs, and does not directly intervene on the RM's training data distribution using counterfactuals to enforce desired robustness properties like invariance. There remains a need for a method that systematically leverages a causal understanding of preference formation to train RMs that are directly sensitive to causal factors and robustly invariant to a wider range of spurious ones.


To address this gap, we propose \textbf{\carma{}} (Causal Attribute-aware Reward Modeling), a novel framework grounded in the explicit causal model of answer generation and evaluation introduced earlier (Section \ref{sec:preliminaries}, Figure \ref{fig:causal_graph}). The core idea of \carma{} is to directly teach the reward model to differentiate between genuine quality drivers and superficial cues by augmenting the standard preference dataset with targeted, LLM-generated counterfactual examples. This involves creating two key types of synthetic training pairs: (1) \textit{Causal Augmentation}, which generates minimally different responses that isolate changes along specific attributes identified as \textit{causal} (like factuality or relevance), thereby explicitly teaching the model sensitivity to genuine quality improvements or degradations. (2) \textit{Neutral Augmentation}, which produces pairs that vary primarily in \textit{spurious} ways (such as style or formatting) while preserving the core causal content, explicitly training the model for invariance to these superficial changes via tie-labels. By training on this enriched dataset using a modified preference loss (detailed in Section \ref{sec:methodology}), \carma{} learns a reward function that aligns more closely with the underlying causal factors of quality. 
Our empirical evaluations demonstrate that \carma{} leads to significantly improved robustness, boosting average accuracy on RewardBench by up to 4.5 percentage points over standard baselines, with significant gains in safety and reasoning capabilities.

The remainder of this paper details our causal framework (Section \ref{sec:preliminaries}), the \carma{} methodology (Section \ref{sec:methodology}), theoretical justifications (Section \ref{sec:theory}), and comprehensive experimental results (Section \ref{sec:experiments}) which address key \hyperref[list:research_questions]{research questions} towards robust reward modeling.


==> archived/notations_20250506.tex <==
\section{Preliminaries and Causal Framework}
\label{sec:preliminaries}

We aim to develop a reward model that accurately assesses the quality of an answer $A$ provided in response to a query $Q$. Our approach is grounded in a causal framework designed to distinguish genuine quality drivers from spurious correlates often present in preference data.

\subsection{Reward Model and Pairwise Preferences}
Let $\hat{R}(Q, A)$ denote the learned reward model, which assigns a scalar score reflecting the quality of answer $A$ for query $Q$. While $\hat{R}$ provides a pointwise score, it is typically trained using pairwise preference data. Given two answers $A_1$ and $A_2$ for the same query $Q$, we relate the reward scores to preference probabilities using the Bradley-Terry model \cite{bradley1952rank}:
\begin{equation}
P(A_1 \succ A_2 | Q; \phi) = \sigmoid(\hat{R}_\phi(Q, A_1) - \hat{R}_\phi(Q, A_2)) = \frac{\exp(\hat{R}_\phi(Q, A_1))}{\exp(\hat{R}_\phi(Q, A_1)) + \exp(\hat{R}_\phi(Q, A_2))}
\label{eq:bt_prob_revised}
\end{equation}
where $\hat{R}_\phi$ explicitly denotes the model parameterized by $\phi$, and $\sigmoid(\cdot)$ is the logistic sigmoid function. The parameters $\phi$ are optimized using a dataset of observed preferences, typically by minimizing the negative log-likelihood based on Eq. \ref{eq:bt_prob_revised}.

\subsection{Causal Graph of Answer Generation and Evaluation}
\label{subsec:causal_graph_revised}

We propose a causal model to analyze the generation and evaluation of answers. The process begins with a query \(Q\), which stimulates a latent \emph{intent} \(\mathcal{I}\)—the core information the generator aims to convey. This intent \(\mathcal{I}\) is then realized as the textual \emph{answer} \(A\). From $A$, we derive two sets of attributes: the \emph{causal attributes} \(C = (C_1,\dots,C_{\ell})\), which represent fundamental quality dimensions like factuality or clarity and serve as the Principal Causal Components driving the reward, and the \emph{spurious attributes} \(SP = (SP_1,\dots,SP_{k})\), such as verbosity or style, which are features potentially correlated with preferences but are not intrinsically determinants of quality for query \(Q\). The idealized \emph{ground-truth reward} \(R\) is assumed to be a function solely of the causal attributes $C$ (and possibly $Q$), formally $R = f(Q, C)$, implying $R$ is conditionally independent of $SP$ given $C$ and $Q$.


We postulate the causal relationships shown in Figure \ref{fig:causal_graph} (conceptual) and described in Table \ref{tab:causal_arrows_revised}.

% Placeholder for Figure - replace with actual figure if needed
\begin{figure}[t!]
\centering
% \includegraphics[width=0.6\textwidth]{your_dag_figure.png} % Or use TikZ
\includegraphics[width=0.8\linewidth]{images/CausalDiagram.pdf}
\caption{Conceptual Causal Graph for Reward Modeling. This will be changed.}
\label{fig:causal_graph}
\end{figure}

\begin{table}[ht!]
\centering
\caption{Interpretation of Causal Arrows in the Assumed DAG}
\label{tab:causal_arrows_revised}
\vspace{1em}
\begin{tabular}{p{3cm} p{9cm}} % Adjusted widths
\toprule
\textbf{Arrow} & \textbf{Interpretation} \\
\midrule
\(Q \;\to\; \mathcal{I}\) & The query shapes the intended content. \\
\(\mathcal{I} \;\to\; A\) & The answer text is generated based on the intent. \\
\(A \;\to\; C\) & The answer text manifests causal quality attributes (e.g., accuracy is determined by the stated facts). \\
\(A \;\to\; SP\) & The answer text also manifests spurious attributes (e.g., formatting, length). \\
\(C \;\to\; R\) & The ground-truth reward $R$ is solely determined by the causal attributes $C$ (given $Q$). \\
\midrule
\multicolumn{2}{p{12cm}}{\textbf{Note:} There is no direct arrow $SP \to R$. The core challenge is that naive training of $\hat{R}$ might induce a spurious dependence on $SP$ because $SP$ and $C$ share a common cause $A$, leading to non-causal correlations in the training data.} \\
\bottomrule
\end{tabular}
\end{table}

The primary challenge is that standard training procedures for $\hat{R}_\phi$ using preference data may inadvertently learn sensitivity to $SP$. Because $A$ generates both $C$ and $SP$, these attributes can be correlated. A model maximizing fit to preference data might exploit the correlation between $SP$ and preference labels, learning a reward function $\hat{R}_\phi$ that depends undesirably on $SP$. Our goal is to train $\hat{R}_\phi$ such that its functional dependence on $A$ is mediated primarily through $C$, making it robust to variations in $SP$.

\subsection{Training Data and Counterfactual Augmentation}
\label{subsec:data_augmentation}

Reward models are typically trained on datasets of pairwise preferences $\mathcal{D}_{pref} = \{(Q^{(i)}, y_w^{(i)}, y_l^{(i)})\}_{i=1}^N$. To mitigate the influence of spurious attributes $SP$ and reinforce the role of causal attributes $C$, we augment $\mathcal{D}_{pref}$ with synthetically generated examples, forming an augmented dataset $\mathcal{D}_{aug}$. This augmentation targets two types of causal enforcement:

\begin{itemize}[itemsep=0pt,left=2pt]
    \item \textbf{Isolating Causal Effects:} We generate pairs of answers $(A, B)$ that differ minimally, ideally only along a single causal attribute $C_j$. For instance, if $B$ represents an improvement in $C_j$ over $A$, the pair $(Q, B, A)$ is added to $\mathcal{D}_{aug}$ with the label $B \succ A$. This forces $\hat{R}_\phi$ to assign higher scores to improvements in causal dimensions.
    \item \textbf{Neutralizing Spurious Effects (Neutrals):} We generate pairs $(A1, A2)$ where $A2$ differs from $A1$ primarily in spurious attributes $SP$ (e.g., through paraphrasing or style transfer that preserves $C$) but is intended to have the same ground-truth quality $R$. These pairs are added to $\mathcal{D}_{aug}$ with a "tie" label ($y=\text{tie}$), encouraging $\hat{R}_\phi(Q, A1) \approx \hat{R}_\phi(Q, A2)$. This promotes invariance to spurious variations.
\end{itemize}
The process involves generating candidate augmentations using LLMs prompted with specific instructions to manipulate attributes (based on identified causal elements, as described later) and filtering them for quality and effectiveness. Training on the combined dataset $\mathcal{D}_{pref} \cup \mathcal{D}_{aug}$ using the pairwise objective derived from Eq. \ref{eq:bt_prob_revised} allows the model to disentangle $C$ from $SP$. The specific generation, filtering, and training procedures are detailed in Section \ref{sec:methodology}. % Link to Methodology

% \paragraph{Notation Summary.} For clarity, Table~\ref{tab:notation_revised} recapitulates the key symbols.

% \begin{table}[h!]
% \centering
% \caption{Key Symbols and Descriptions (Revised)}
% \label{tab:notation_revised}
% \vspace{1em}
% \begin{tabular}{ll}
% \toprule
% \textbf{Symbol} & \textbf{Meaning} \\
% \midrule
% \(Q\) & Query or user prompt \\
% \(\mathcal{I}\) & Latent intent (unobserved) \\
% \(A\), \(A_1, A_2\) & Candidate answer(s) in response to \(Q\) \\
% \(C = (C_1,\dots,C_{\ell})\) & Vector of Causal attributes of \(A\) \\
% \(SP = (SP_1,\dots,SP_{k})\) & Vector of Spurious attributes of \(A\) \\
% \(R\) & Ground-truth (ideal) reward, function of $Q, C$ \\
% \(\hat{R}_\phi(Q,A)\) & Learned reward model score, parameterized by $\phi$ \\
% $\mathcal{D}_{pref}$ & Human feedback dataset (pairwise preferences) \\
% $\mathcal{D}_{aug}$ & Augmented dataset (causal/neutral pairs) \\
% $P(A_1 \succ A_2 | Q; \phi)$ & Modeled preference probability using $\hat{R}_\phi$ \\
% \bottomrule
% \end{tabular}
% \end{table}

==> archived/np_20250510.tex <==
\section{Causal Framework for Reward Modeling}
\label{sec:preliminaries}

We aim to develop a reward model that accurately assesses the quality of an answer $\mathrm{A}$ provided in response to a query $\mathrm{Q}$. Our approach is grounded in a causal framework designed to distinguish genuine quality drivers from spurious correlates often present in preference data.

\subsection{Reward Model and Pairwise Preferences}
Let $\hat{\mathrm{R}}(\mathrm{Q}, \mathrm{A})$ denote the learned reward model, which assigns a scalar score reflecting the quality of answer $\mathrm{A}$ for query $\mathrm{Q}$. While $\hat{\mathrm{R}}$ provides a pointwise score, it is typically trained using pairwise preference data. Given two answers $\mathrm{A}_1$ and $\mathrm{A}_2$ for the same query $\mathrm{Q}$, we relate the reward scores to preference probabilities using the Bradley-Terry model \citep{bradley1952rank}:
\begin{equation}
\mathrm{P}(\mathrm{A}_1 \succ \mathrm{A}_2 | \mathrm{Q}; \theta) = \sigmoid(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2)) = \frac{\exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1))}{\exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1)) + \exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2))}
\label{eq:bt_prob_roman}
\end{equation}
where $\hat{\mathrm{R}}_\theta$ explicitly denotes the model parameterized by $\theta$, and $\sigmoid(\cdot)$ is the logistic sigmoid function. The parameters $\theta$ are optimized using a dataset of observed preferences $\mathcal{D}_{\mathrm{pref}} = \{(\mathrm{Q}^{(i)}, \mathrm{y}_w^{(i)}, \mathrm{y}_l^{(i)})\}_{i=1}^N$, typically by minimizing the negative log-likelihood based on Eq. \ref{eq:bt_prob_roman}.

\subsection{Causal Framework for Reward Modeling}
\label{subsec:causal_graph}

We propose a causal model (Figure \ref{fig:causal_graph}) to analyze the generation and evaluation of answers. The process begins with a query $\mathrm{Q}$, which stimulates a latent \textit{intent} $\mathcal{I}$. We define \textit{Intent} $\mathcal{I}$ as an unobserved latent variable representing the core, high-quality information and goals the generator (human or LLM) aims to convey in response to $\mathrm{Q}$, before stylistic choices or other potentially spurious elements arise in the final textual manifestation. This intent $\mathcal{I}$ is then realized as the textual answer $\mathrm{A}$.

From the answer $\mathrm{A}$, we derive two sets of attributes:
\begin{itemize}[itemsep=0pt,left=0pt]
    \item \textbf{Causal Attributes} $\mathrm{C}(\mathrm{A}) = \{\mathrm{C}_1(\mathrm{A}), \dots, \mathrm{C}_\ell(\mathrm{A})\}$: These are the \textit{Principal Causal Components} representing fundamental quality dimensions (e.g., factuality, relevance, safety) that genuinely determine the response's quality relative to the query $\mathrm{Q}$.
    \item \textbf{Spurious Attributes} $\mathrm{SP}(\mathrm{A}) = \{\mathrm{SP}_1(\mathrm{A}), \dots, \mathrm{SP}_k(\mathrm{A})\}$: These are features (e.g., length, formatting, politeness, specific phrasing) that might be statistically correlated with human preferences in $\mathcal{D}_{\mathrm{pref}}$ but do not intrinsically determine the answer's true quality. We note that the set of all spurious features is (a) greater than the causal feature set and (b) \emph{not} known a priori, and hence directly controlling for them is challenging.
\end{itemize}
We assume an idealized \textit{ground-truth reward} $\mathrm{R}^*(\mathrm{Q}, \mathrm{A})$ exists, which is a function solely of the query and the causal attributes: $\mathrm{R}^*(\mathrm{Q}, \mathrm{A}) = f^*(\mathrm{Q}, \mathrm{C}(\mathrm{A}))$. This implies $\mathrm{R}^*$ is conditionally independent of $\mathrm{SP}(\mathrm{A})$ given $\mathrm{Q}$ and $\mathrm{C}(\mathrm{A})$. The causal relationships are depicted in Figure \ref{fig:causal_graph} and interpreted in Table \ref{tab:causal_arrows}.

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{images/causalDiagram.pdf} 
\caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query, $\mathcal{I}$ is the latent intent for the response, $\mathcal{U}$ is the set of unknown confounders from the generator, $\mathrm{A}$ is the generated answer, $\mathrm{C}(\mathrm{A})$ are causal attributes, $\mathrm{SP}(\mathrm{A})$ are spurious attributes, and $\mathrm{R}$ is the ground-truth reward. The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}$, such that $\mathrm{SP}(\mathrm{A})$ is conditionally independent of $\mathrm{R}$ given $\mathrm{C}(\mathrm{A})$ and $\mathrm{Q}$.}
\label{fig:causal_graph}
\end{figure}

\begin{table}[ht!]
\centering
\caption{Interpretation of Causal Arrows in the Assumed DAG}
\label{tab:causal_arrows}
\vspace{1em}
\begin{tabular}{p{3cm} p{9cm}} % Adjusted widths
\toprule
\textbf{Arrow} & \textbf{Interpretation} \\
\midrule
$\mathrm{Q} \;\to\; \mathcal{I}$ & The query shapes the generator's intent. \\
$\mathcal{I}, \mathcal{U} \;\to\; \mathrm{A}$ & The answer text is generated based on the intent but is shaped by the generator's internal latent state. \\$\mathrm{A} \;\to\; \mathrm{C}(\mathrm{A})$ & The answer text manifests causal quality attributes. \\
$\mathrm{A} \;\to\; \mathrm{SP}(\mathrm{A})$ & The answer text also manifests spurious attributes. \\
$\mathrm{C}(\mathrm{A}) \;\to\; \mathrm{R}$ & The ground-truth reward $\mathrm{R}$ is solely determined by the causal attributes $\mathrm{C}(\mathrm{A})$ (given $\mathrm{Q}$). \\
\midrule
\multicolumn{2}{p{12cm}}{\textbf{Note:} There is no direct arrow $\mathrm{SP}(\mathrm{A}) \to \mathrm{R}$. The challenge is that standard training of $\hat{\mathrm{R}}_\theta$ on $\mathcal{D}_{\mathrm{pref}}$ might induce a spurious dependence on $\mathrm{SP}(\mathrm{A})$ because $\mathrm{SP}(\mathrm{A})$ and $\mathrm{C}(\mathrm{A})$ share a common cause $\mathrm{A}$, leading to non-causal correlations between $\mathrm{SP}(\mathrm{A})$ and preference labels derived from $\mathrm{R}^*$.} \\
\bottomrule
\end{tabular}
\end{table}

The primary challenge arises because standard training procedures for $\hat{\mathrm{R}}_\theta$ may inadvertently learn sensitivity to $\mathrm{SP}(\mathrm{A})$ due to correlations present in $\mathcal{D}_{\mathrm{pref}}$. Since $\mathrm{A}$ generates both $\mathrm{C}(\mathrm{A})$ and $\mathrm{SP}(\mathrm{A})$, these attributes can be statistically associated. A model $\hat{\mathrm{R}}_\theta$ optimized solely to fit observed preferences might exploit the correlation between $\mathrm{SP}(\mathrm{A})$ and preference labels, leading to undesirable dependencies. Our goal is to train $\hat{\mathrm{R}}_\theta$ such that its functional dependence on $\mathrm{A}$ is primarily mediated through the causal attributes $\mathrm{C}(\mathrm{A})$, rendering it robust to variations in the spurious attributes $\mathrm{SP}(\mathrm{A})$.

\subsection{Counterfactuals via Causal Interventions}
\label{subsec:interventions}

To instill causal awareness and robustness in $\hat{\mathrm{R}}_\theta$, we leverage the concept of causal interventions \citep{pearl2009causality}, formally denoted by the $do(\cdot)$ operator. An intervention $do(X=x)$ represents setting a variable $X$ to a specific value $x$, potentially breaking its dependence on its usual causes. In our context, we consider hypothetical interventions on the attributes of an answer $\mathrm{A}$. For instance, $A_{do(\mathrm{C}_i=c)}$ represents the ideal counterfactual answer that would manifest if the $i$-th causal attribute $\mathrm{C}_i$ were set to value $c$, while all other causal attributes $\mathrm{C}_{j \neq i}$ and all spurious attributes $\mathrm{SP}$ remained unchanged from their original values in $\mathrm{A}$. Similarly, $A_{do(\mathrm{SP}=sp')}$ would be the result of altering only the spurious attributes to $sp'$, holding $\mathrm{C}(\mathrm{A})$ constant, and $A_{do(\mathrm{C}=\mathbf{c}')}$ represents intervening on the entire vector of causal attributes.

Since we cannot perform these ideal interventions directly on generated text, we use Large Language Models (LLMs) to approximate them. We prompt an LLM to rewrite an existing answer $\mathrm{A}$ according to specific instructions aimed at modifying a target attribute (e.g., setting $\mathrm{C}_i$ to 1 or 0) while explicitly instructing the LLM to preserve all other aspects ("minimal change"). We denote these LLM-generated approximations of counterfactuals as $\tilde{\mathrm{A}}_{do(\cdot)}$. The CARMA methodology relies on strategically generating and utilizing these imperfect counterfactuals within the training process.

\subsection{Augmented Training Data for Causal Disentanglement}
\label{subsec:data_augmentation}

\begin{table}[!thbp]
\centering
\caption{Summary of Synthetic Data Augmentation Strategies in CARMA.}
\label{tab:augmentation_summary}
\vspace{1em} % space between caption and table
%  column widths
\newcolumntype{L}{>{\raggedright\arraybackslash}p{2.5cm}} % Left-aligned paragraph
\newcolumntype{P}{>{\raggedright\arraybackslash}p{4.5cm}} % Left-aligned paragraph for pairs
\newcolumntype{C}{>{\centering\arraybackslash}p{1.3cm}}  % Centered paragraph
\newcolumntype{R}{>{\raggedleft\arraybackslash}p{2.2cm}}   % Right-aligned paragraph

\begin{tabular}{@{}l L P C R@{}}
\toprule
\textbf{Category} & \textbf{Strategy} & \textbf{Generation Pair Example} & \textbf{Assigned Label} & \textbf{Training Objective ($\mathrm{P}_\theta$)} \\
\midrule
\multicolumn{5}{l}{\textit{Causal Augmentation ($\mathcal{D}_{\mathrm{causal}}$) - Enhancing Sensitivity to C}} \\
\midrule
Causal & Attribute Upgradation & $(\tilde{\mathrm{A}}_{do(\mathrm{C}_j=1)}, \mathrm{A})$ & $\tilde{\mathrm{A}} \succ \mathrm{A}$ & $\to 1$ \\
Causal & Attribute Degradation & $(\mathrm{A}, \tilde{\mathrm{A}}_{do(\mathrm{C}_j=0)})$ & $\mathrm{A} \succ \tilde{\mathrm{A}}$ & $\to 1$ \\
Causal & Relevance Contrast & $(\mathrm{A}_1, \mathrm{B}_2)$ \newline \footnotesize{where $\mathrm{C}(\mathrm{A}_1)\neq \mathbf{0}, \mathrm{C}(\mathrm{B}_2)=\mathbf{0}$} & $\mathrm{A}_1 \succ \mathrm{B}_2$ & $\to 1$ \\
\midrule
\multicolumn{5}{l}{\textit{Neutral Augmentation ($\mathcal{D}_{\mathrm{neutral}}$) - Enforcing Invariance to SP}} \\
\midrule
Neutral & Causally-Aligned Reconstruction & $(\mathrm{A}_1, \tilde{\mathrm{A}}_{2, do(\mathrm{C}=\mathrm{C}(\mathrm{A}_1))})$ \newline and symmetric pair for $\mathrm{A}_2$  & $ \approx $ (tie) & $\approx 0.5$ \\
Neutral & Spurious Feature Perturbation & $(\mathrm{A}, \tilde{\mathrm{A}}_{do(\mathrm{SP}=sp')})$ & $ \approx $ (tie) & $\approx 0.5$ \\
Neutral & Irrelevant Pair Comparison & $(\mathrm{B}_1, \mathrm{B}_2)$ \newline \footnotesize{where $\mathrm{C}(\mathrm{B}_1)=\mathrm{C}(\mathrm{B}_2)=\mathbf{0}$} & $ \approx $ (tie) & $\approx 0.5$ \\
\bottomrule
\end{tabular}
\end{table}


We augment the original preference dataset $\mathcal{D}_{\mathrm{pref}}$ with synthetically generated examples $\mathcal{D}_{\mathrm{aug}}$ designed to enforce specific causal properties on $\hat{\mathrm{R}}_\theta$. This augmented dataset $\mathcal{D}_{\mathrm{aug}}$ comprises two principal categories: Causal Augmentation Pairs ($\mathcal{D}_{\mathrm{causal}}$) and Neutral Augmentation Pairs ($\mathcal{D}_{\mathrm{neutral}}$).

\subsubsection{Causal Augmentation Pairs (\texorpdfstring{$\mathcal{D}_{\mathrm{causal}}$}{D-causal})}
These pairs are designed to explicitly teach $\hat{\mathrm{R}}_\theta$ sensitivity to changes in the principal causal attributes $\mathrm{C}(\mathrm{A})$. They are incorporated into the standard preference loss term.

\paragraph{1. Attribute Isolation via Intervention.}
For an original answer $\mathrm{A}$ (drawn from $\mathcal{D}_{\mathrm{pref}}$, being either $\mathrm{y}_w^{(i)}$ or $\mathrm{y}_l^{(i)}$) and a specific causal attribute $\mathrm{C}_j$, we generate LLM-approximated counterfactuals $\tilde{\mathrm{A}}_{do(\mathrm{C}_j=c)}$. If $\mathrm{A}$ is a preferred answer ($\mathrm{y}_w^{(i)}$), we generate its degraded version $\tilde{\mathrm{A}}_{do(\mathrm{C}_j=0)}$ and add the pair $(\mathrm{A}, \tilde{\mathrm{A}}_{do(\mathrm{C}_j=0)})$ to $\mathcal{D}_{\mathrm{causal}}$ with the preference label $\mathrm{A} \succ \tilde{\mathrm{A}}_{do(\mathrm{C}_j=0)}$. If $\mathrm{A}$ is a rejected answer ($\mathrm{y}_l^{(i)}$), we generate its upgraded version $\tilde{\mathrm{A}}_{do(\mathrm{C}_j=1)}$ and add the pair $(\tilde{\mathrm{A}}_{do(\mathrm{C}_j=1)}, \mathrm{A})$ to $\mathcal{D}_{\mathrm{causal}}$ with the label $\tilde{\mathrm{A}}_{do(\mathrm{C}_j=1)} \succ \mathrm{A}$. Training on these pairs forces the model $\hat{\mathrm{R}}_\theta$ to assign higher scores to responses with improvements along individual causal dimensions, satisfying $P_\theta(\mathrm{A} \succ \tilde{\mathrm{A}}_{do(\mathrm{C}_j=0)}) \to 1$ and $P_\theta(\tilde{\mathrm{A}}_{do(\mathrm{C}_j=1)} \succ \mathrm{A}) \to 1$.

\paragraph{2. Relevance Contrast Augmentation.}
To further reinforce the importance of overall causal quality, we create pairs contrasting relevant and irrelevant answers. For a preferred answer $\mathrm{A}_1 = \mathrm{y}_w^{(i)}$ from $\mathcal{D}_{\mathrm{pref}}$ (assumed to be causally relevant, i.e., $\mathrm{C}(\mathrm{A}_1) \neq \mathbf{0}$) and an answer $\mathrm{B}_2$ known to be irrelevant to the query $\mathrm{Q}^{(i)}$ (i.e., $\mathrm{C}(\mathrm{B}_2) = \mathbf{0}$, such as an answer from a different query), we add the pair $(\mathrm{A}_1, \mathrm{B}_2)$ to $\mathcal{D}_{\mathrm{causal}}$ with the label $\mathrm{A}_1 \succ \mathrm{B}_2$. This encourages the model to strongly prefer relevant answers over irrelevant ones, driving $P_\theta(\mathrm{A}_1 \succ \mathrm{B}_2) \to 1$.

\subsubsection{Neutral Augmentation Pairs (\texorpdfstring{$\mathcal{D}_{\mathrm{neutral}}$}{D-neutral})}
These pairs are designed to teach $\hat{\mathrm{R}}_\theta$ invariance to spurious attributes $\mathrm{SP}(\mathrm{A})$ when the causal attributes $\mathrm{C}(\mathrm{A})$ are held constant. They are assigned a "tie" label ($y=\text{tie}$) and are handled by a specific term in the loss function (Section \ref{subsec:training_phase}), encouraging $\hat{\mathrm{R}}_\theta(\mathrm{A}_1) \approx \hat{\mathrm{R}}_\theta(\mathrm{A}_2)$ for neutral pairs $(\mathrm{A}_1, \mathrm{A}_2)$.

\paragraph{1. Causally-Aligned Reconstruction.}
Given an original preference pair $(\mathrm{A}_1, \mathrm{A}_2)$ from $\mathcal{D}_{\mathrm{pref}}$ with $\mathrm{A}_1 \succ \mathrm{A}_2$, we first identify the difference in their causal attribute profiles $\Delta \mathrm{C} = \mathrm{C}(\mathrm{A}_1) - \mathrm{C}(\mathrm{A}_2)$ (using an LLM analysis based on the identified attributes and causal elements). We then prompt the LLM to rewrite $\mathrm{A}_2$ to match the causal profile of $\mathrm{A}_1$, yielding an approximation $\tilde{\mathrm{A}}_{2, do(\mathrm{C} = \mathrm{C}(\mathrm{A}_1))}$. The prompt instructs the LLM to preserve the original spurious characteristics (style, formatting) of $\mathrm{A}_2$ during this rewrite. The pair $(\mathrm{A}_1, \tilde{\mathrm{A}}_{2, do(\mathrm{C} = \mathrm{C}(\mathrm{A}_1))})$ is added to $\mathcal{D}_{\mathrm{neutral}}$ with $y=\text{tie}$. A symmetric pair $(\mathrm{A}_2, \tilde{\mathrm{A}}_{1, do(\mathrm{C} = \mathrm{C}(\mathrm{A}_2))})$ is also generated and added. Training on these encourages $P_\theta(\mathrm{A}_1 \succ \tilde{\mathrm{A}}_{2, do(\mathrm{C}=\mathrm{C}(\mathrm{A}_1))}) \approx 0.5$.

\paragraph{2. Spurious Feature Perturbation.}
For an original answer $\mathrm{A}$, we generate an approximation $\tilde{\mathrm{A}}_{do(\mathrm{SP}=sp')}$ by applying a meaning-preserving transformation that primarily affects spurious attributes $\mathrm{SP}$ while holding causal attributes $\mathrm{C}$ constant (e.g., paraphrasing, changing list format to paragraph format). The pair $(\mathrm{A}, \tilde{\mathrm{A}}_{do(\mathrm{SP}=sp')})$ is added to $\mathcal{D}_{\mathrm{neutral}}$ with $y=\text{tie}$, encouraging $P_\theta(\mathrm{A} \succ \tilde{\mathrm{A}}_{do(\mathrm{SP}=sp')}) \approx 0.5$.

\paragraph{3. Irrelevant Pair Comparison.}
We select two answers, $\mathrm{B}_1$ and $\mathrm{B}_2$, both irrelevant to the query $\mathrm{Q}$ (ideally $\mathrm{C}(\mathrm{B}_1) = \mathrm{C}(\mathrm{B}_2) = \mathbf{0}$), which may differ arbitrarily in their spurious attributes $\mathrm{SP}(\mathrm{B}_1)$ and $\mathrm{SP}(\mathrm{B}_2)$. The pair $(\mathrm{B}_1, \mathrm{B}_2)$ is added to $\mathcal{D}_{\mathrm{neutral}}$ with $y=\text{tie}$. This reinforces that irrelevant responses should receive similar (low) scores regardless of their spurious features, encouraging $P_\theta(\mathrm{B}_1 \succ \mathrm{B}_2) \approx 0.5$.

The specific LLM prompts used to implement these generation strategies are detailed in Appendix \ref{sec:prompt_templates}. The combined dataset $\mathcal{D} = \mathcal{D}_{\mathrm{pref}} \cup \mathcal{D}_{\mathrm{causal}} \cup \mathcal{D}_{\mathrm{neutral}}$ (after filtering, see Section \ref{subsec:filtering_appendix}) provides the necessary signal to train a causally robust reward model.
The crucial insight that we want to leave the reader with, is that a reward model learns to disentangle causal attributes from spurious ones, only when shown examples of such disentanglement.

==> archived/np_20250516.tex <==

% \vspace{-0.15in}
\section{Causal Framework for Reward Modeling}
\label{sec:preliminaries}

% \vspace{-0.1in}
% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{images/causalDiagram.pdf} 
% \caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query, $\mathcal{I}$ is the latent intent for the response, $\mathcal{U}$ is the set of unknown confounders from the generator, $\mathrm{A}$ is the generated answer, $\mathrm{C}(\mathrm{A})$ are causal attributes, $\mathrm{SP}(\mathrm{A})$ are spurious attributes, and $\mathrm{R}^*$ is the ground-truth reward. The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, such that its dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$.}
% \label{fig:causal_graph}
% \end{figure}

\vspace{-0.1in}
\begin{figure}[t!]
\centering
\includegraphics[width=0.7\linewidth]{images/CausalGraphA.pdf} 
\caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query. The Answer (A) comprises of two types of attributes, $\mathrm{C}(\mathrm{A})$, which are causal attributes, and $\mathrm{SP}(\mathrm{A})$ which are spurious attributes. $\mathrm{R}^*$ is the human annotated or ground-truth reward which are posited to depend only on C(A). The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, such that its dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$. \vspace{-0.2in}}
\label{fig:causal_graph}
\end{figure}


% \begin{figure}[!t]               % one float, two columns inside
%   \centering
%   \begin{minipage}[t]{0.62\textwidth}
%     \vspace{0.0in}
%     \centering
%     \includegraphics[width=\linewidth]{images/CausalGraphA.pdf}
%     \vspace{-0.25in}
%     \captionof{figure}{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query. Answer (A) has causal attributes $\mathrm{C}(\mathrm{A})$ and spurious attributes $\mathrm{SP}(\mathrm{A})$. Ground-truth reward $\mathrm{R}^*$ depends only on $\mathrm{C(A)}$ and $\mathrm{Q}$. Goal: train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, primarily via $\mathrm{C}(\mathrm{A})$. Augmentations heighten $\hat{\mathrm{R}}_\theta$'s sensitivity to $\mathrm{C(A)}$ (approximated by oracle LLM).}
%     \label{fig:causal_graph}
%   \end{minipage}
%   \begin{minipage}[t]{0.34\textwidth}
%         \centering
%         \vspace{-0.2in}
%         \resizebox{\linewidth}{!}{% Make table fit the minipage width
%         \begin{tabular}{c|p{0.8\linewidth}} % Adjusted p{} width relative to table
%         \toprule
%         \textbf{Path} & \textbf{Interpretation} \\ % Changed Arrow to Path
%         \midrule
%         $(\mathrm{Q}, \mathrm{C}(\mathrm{A})) \;\to\; \mathrm{R}^*$ & $\mathrm{R}^*$ is solely determined by causal attributes $\mathrm{C(A)}$ and question $\mathrm{Q}$, stable across labelers. \\
%         $\mathrm{Q}\leftrightarrow \mathrm{SP(A)}$  & $\mathrm{SP(A)}$ (unknown spurious attributes not in $\mathrm{C(A)}$) are correlated/confounded with $\mathrm{Q}$ via unknown, unstable factors.  \\
%         $\mathrm{Q}\rightarrow \mathrm{C(A)}$ & $\mathrm{Q}$ determines relevant causal attributes $\mathrm{C(A)}$ for the reward. \\
%         $\mathrm{SP(A)} \leftrightarrow \mathrm{C(A)}$ & Causal and spurious attributes are bidirectionally related (e.g., some $\mathrm{SP(A)}$ may or may not have parents in $\mathrm{C(A)}$). \\
%         \midrule
%         \bottomrule
%         \end{tabular}
%         } % End resizebox
%         \vspace{-0.1in}
%         \caption{$\mathrm{R^*} \perp \mathrm{SP(A)} | \mathrm{C(A)}$. $\mathrm{SP(A)}$ is unknown and high-dimensional.\vspace{-0.2in}}
%         \label{tab:causal_arrows}
%   \end{minipage}\hfill          % \hfill inserts a flexible gutter
  
% \end{figure}
%   \vspace{0.03in}


% \vspace{-0.1in}
% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{images/CausalGraphNew.pdf} 
% \caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query, $\mathcal{I}$ is the latent intent for the response, $\mathcal{U}$ is the set of unknown confounders from the generator, $\mathrm{A}$ is the generated answer, $\mathrm{C}(\mathrm{A})$ are causal attributes, $\mathrm{SP}(\mathrm{A})$ are spurious attributes, and $\mathrm{R}^*$ is the ground-truth reward. The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, such that its dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$.}
% \label{fig:causal_graph}
% \end{figure}

\vspace{-0.05in}
We aim to develop a reward model that accurately assesses the quality of an answer $\mathrm{A}$ provided in response to a query $\mathrm{Q}$. Our approach is grounded in a causal framework designed to distinguish genuine quality drivers from spurious correlates often present in preference data. This involves understanding the answer generation process and then strategically augmenting training data with approximated counterfactual examples.

\vspace{-0.05in}
\subsection{Reward Model and Pairwise Preferences}
We train a reward model (RM), denoted $\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A})$, to assign a scalar quality score to an answer $\mathrm{A}$ for a query $\mathrm{Q}$. This RM is typically optimized on a dataset  preferences pairs $\mathcal{D}_{\mathrm{pref}} = \{(\mathrm{Q}^{(i)}, \mathrm{y}_w^{(i)}, \mathrm{y}_l^{(i)})\}_{i=1}^N$. Given a pair of answers $(\mathrm{A}_1, \mathrm{A}_2)$, the probability of $\mathrm{A}_1$ being preferred over $\mathrm{A}_2$ is commonly modeled using the Bradley-Terry framework \citep{bradley1952rank}:
\begin{equation}
\mathrm{P}(\mathrm{A}_1 \succ \mathrm{A}_2 | \mathrm{Q}; \theta) = \sigmoid(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{s}_\theta(\mathrm{Q}, \mathrm{A}_2)) = \frac{\exp(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1))}{\exp(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1)) + \exp(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_2))}
\label{eq:bt_prob_roman}
\end{equation}
where $\hat{s}_\theta(\mathrm{Q}, \mathrm{A})$ represents the underlying scalar score (or logit) assigned by the model to answer $\mathrm{A}$ for query $\mathrm{Q}$.\footnote{The score $\hat{s}_\theta(\mathrm{Q}, \mathrm{A})$ can be the direct output of a reward head or, in some pairwise preference models, $\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{s}_\theta(\mathrm{Q}, \mathrm{A}_2)$ might be directly modeled as the logit of preferring $\mathrm{A}_1$ over $\mathrm{A}_2$.} The parameters $\theta$ are learned by minimizing the negative log-likelihood of observed preferences.

% \subsection{Reward Model and Pairwise Preferences}
% Let $\hat{\mathrm{R}}(\mathrm{Q}, \mathrm{A})$ denote the learned reward model, which assigns a scalar score reflecting the quality of answer $\mathrm{A}$ for query $\mathrm{Q}$. While $\hat{\mathrm{R}}$ provides a pointwise score, it is typically trained using pairwise preference data. Given two answers $\mathrm{A}_1$ and $\mathrm{A}_2$ for the same query $\mathrm{Q}$, we relate the reward scores to preference probabilities using the Bradley-Terry model \citep{bradley1952rank}:
% \begin{equation}
% \mathrm{P}(\mathrm{A}_1 \succ \mathrm{A}_2 | \mathrm{Q}; \theta) = \sigmoid(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2)) = \frac{\exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1))}{\exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1)) + \exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2))}
% \label{eq:bt_prob_roman}
% \end{equation}
% where $\hat{\mathrm{R}}_\theta$ explicitly denotes the model parameterized by $\theta$, and $\sigmoid(\cdot)$ is the logistic sigmoid function. The parameters $\theta$ are optimized using a dataset of observed preferences $\mathcal{D}_{\mathrm{pref}} = \{(\mathrm{Q}^{(i)}, \mathrm{y}_w^{(i)}, \mathrm{y}_l^{(i)})\}_{i=1}^N$, typically by minimizing the negative log-likelihood based on Eq. \ref{eq:bt_prob_roman}.



\subsection{A Causal Model of Answer Generation}
\label{subsec:causal_graph}



We propose a causal model (Figure \ref{fig:causal_graph}) to analyze the generation of answers and how their quality is perceived. The process begins with a query, answer pair $\mathrm{Q},\mathrm{A}$ that is rated by a human or some other agent providing ground truth reward label. {\color{blue} The answer has two parts, one being causal attributes ($C(A)$) and the other being spurious attributes ($SP(A)$). The reward labeler (or human) uses causal attributes ($C(A)$) to provide ground truth reward label that is part of the training data. All other features are considered to be $SP(A)$ and are correlated with $C(A)$. Further, at the time of answer generation, there may be unknown factors (additional prompts to condition the answer, or unknown exogenous confounding factors) that correlate spurious factors $SP(A)$ with the question. 
We assume the following: \textit{If the entire process is repeated with different labeler and answer generator, then $Q, C(A) \rightarrow R^{*}$ relationship of reward labeling  is stable/invariant compared to unstable correlation between spurious factors and the question.}}

We formalize this below. We have two sets of attributes that constitute the answer:
\begin{itemize}[itemsep=0pt,left=0pt]
    \item \textbf{Causal Attributes} $\mathrm{C}(\mathrm{A}) = \{\mathrm{C}_1(\mathrm{A}), \dots, \mathrm{C}_\ell(\mathrm{A})\}$: These are the \textit{Principal Causal Components} representing fundamental quality dimensions (e.g., factuality, relevance, safety) that genuinely determine the reward label of the answer relative to the query $\mathrm{Q}$.
    \item \textbf{Spurious Attributes} $\mathrm{SP}(\mathrm{A}) = \{\mathrm{SP}_1(\mathrm{A}), \dots, \mathrm{SP}_k(\mathrm{A})\}$: These are features (e.g., length, formatting, politeness, specific phrasing) that might be statistically correlated with human preferences and exhibit a correlation with the query in $\mathcal{D}_{\mathrm{pref}}$ but do not intrinsically determine the reward label of the answer.
\end{itemize}
We assume an idealized \textit{ground-truth reward} $\mathrm{R}^*(\mathrm{Q}, \mathrm{A})$ exists, which is a function solely of the query and the causal attributes: $\mathrm{R}^*(\mathrm{Q}, \mathrm{A}) = f^*(\mathrm{Q}, \mathrm{C}(\mathrm{A}))$. 

This implies $\mathrm{R}^*$ is conditionally independent of $\mathrm{SP}(\mathrm{A})$ given $\mathrm{Q}$ and $\mathrm{C}(\mathrm{A})$. The causal relationships are depicted in Figure \ref{fig:causal_graph} and interpreted in Table \ref{tab:causal_arrows}.The primary challenge arises because standard training procedures for $\hat{\mathrm{R}}_\theta$ may inadvertently have higher sensitivity to $\mathrm{SP}(\mathrm{A})$ due to it being high dimensional (and unknown). Our goal is to train $\hat{\mathrm{R}}_\theta$ such that its functional dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$, rendering it robust to variations in $\mathrm{SP}(\mathrm{A})$.



\begin{table}[t!]
\centering
\caption{Explanation of the Causal Model}
\label{tab:causal_arrows}
\vspace{1em}
\begin{tabular}{c|p{9cm}} % Adjusted widths
\toprule
\textbf{Arrow} & \textbf{Interpretation} \\
\midrule
$(\mathrm{Q}, \mathrm{C}(\mathrm{A})) \;\to\; \mathrm{R}^*$ & The ground-truth reward $\mathrm{R}^*$ is solely determined by the causal attributes $\mathrm{C(A)}$ and the question $\mathrm{Q}$. The labeling agent is looks  at only $\mathrm{C(A)}$ and $\mathrm{Q}$ to decide on the label. This relationships is assumed to be stable across labeling agents. \\
$\mathrm{Q}\leftrightarrow \mathrm{SP(A)}$  & $\mathrm{SP(A)}$ - all unknown spurious attributes that is not $\mathrm{C(A)}$ but correlated/confounded with question through unknown factors. This correlation is unstable and is different depending on other exogenous factors.  \\
$\mathrm{Q}\rightarrow \mathrm{C(A)}$ & Question determines causal attributes of the answer relevant to the reward \\
$\mathrm{SP(A)} \leftrightarrow \mathrm{C(A)}$ & Causal and spurious attributes have bidirectional relationship. Specifically we will model $SP_1(A) \subseteq SP(A)$ that has no parents in $C(A)$, and $SP_2(A) \subset SP(A)$ with direct parents in $C(A)$ \\

%$\mathrm{A} \;\to\; \mathrm{C}(\mathrm{A})$ & The answer text manifests causal quality attributes. \\
%$\mathrm{A} \;\to\; \mathrm{SP}(\mathrm{A})$ & The answer text also manifests spurious attributes. \\
\midrule
\multicolumn{2}{p{12cm}}{\textbf{Note:} Key property is the conditional independence $\mathrm{R^*} \perp \mathrm{SP(A)} | \mathrm{C(A)}$. $\mathrm{SP(A)}$ is unknown and potentially very high dimensional ($k >> \ell$). Our augmentation strategies are aimed at heightening sensitivity of reward to $\mathrm{C(A)}$ by varying answers along these only. An approximation to $\mathrm{C(A)}$ is obtained by querying an oracle LLM.  } \\
\bottomrule
\end{tabular}
\end{table} 



\vspace{-0.05in}
\subsection{Construction of Counterfactuals when causal attributes change}
\label{subsec:approximating_counterfactuals}

\vspace{-0.05in}
{\color{blue}
To train $\hat{\mathrm{R}}_\theta$ for causal sensitivity and spurious invariance, we leverage the concept of counterfactuals: reasoning about how an answer's quality would change if specific attributes were altered. Given an answer $\mathrm{A}$ with attributes $(\mathrm{C}(\mathrm{A}), \mathrm{SP}(\mathrm{A}))$, an ideal counterfactual $A_{(C_j \leftarrow c'_j)} (u)$ would represent $\mathrm{A}$ with only its $j$-th causal attribute $C_j$ changed to $c'_j$ and its effect on other features through their causal relationships, given all else (all hidden factors of variation captured in variable $u$) held in those values that would give rise to the factual answer. Formally, the counterfactual is sampled from $P_{U}(A_{(C_j \leftarrow c'_j)} (U) | A(U) =a)$ - a counterfactual distribution under the exogenous conditional distribution $u$ that gives rise to the factual answer $a$ and under the intervention $(C_j \leftarrow c'_j)$.

Perfectly constructing such ideal textual counterfactuals is intractable. \carma{} therefore employs Large Language Models (LLMs) to \textit{generate new answers}, denoted $\tilde{\mathrm{A}}_{(\cdot)}$, that \textit{approximate} these ideal counterfactuals. For example, $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})}(u)$ is an LLM rewrite of the original answer $\mathrm{A}$, prompted to degrade $C_j$, in the sense of lowering the reward, while minimally affecting other attributes. }

{\color{blue}
\begin{remark} For the sake of brevity in what follows, we use $\tilde{A}_{C_j \leftarrow c}$ dropping the dependence on exogenous condition $u$ sampled under condition $A(u) = a$. We assume that the generated answer approximately reflects such a sample. While these are approximations and perfect attribute isolation is difficult, they provide the targeted variations necessary for our data augmentation.
\end{remark}
}
% \begin{remark}
% In \carma{}, attributes are identified from an existing answer $\mathrm{A}$. An LLM then constructs a \textit{new textual instance} $\tilde{\mathrm{A}}^{(\cdot)}$ to approximate a desired counterfactual state (e.g., $C_j$ modified). 
% \end{remark}

% \subsection{Approximating Counterfactual Answer Variations}
% \label{subsec:approximating_counterfactuals}

% To teach $\hat{\mathrm{R}}_\theta$ the desired sensitivities and invariances, we reason about \textit{counterfactual answers}: what an answer \textit{would have been like} if certain attributes had been different. Given an original answer $\mathrm{A}$ (with its observed attributes $\mathrm{C}(\mathrm{A})$ and $\mathrm{SP}(\mathrm{A})$), we consider an ideal counterfactual, such as $A^{(C_j \leftarrow c'_j)}$, where only the $j$-th causal attribute $C_j$ is hypothetically changed to $c'_j$, while all other causal attributes $\mathrm{C}_{k \neq j}(\mathrm{A})$ and all spurious attributes $\mathrm{SP}(\mathrm{A})$ are held constant.

% Directly constructing such ideal counterfactual answers from a given text $\mathrm{A}$ while perfectly isolating attribute changes is generally intractable. \carma{} employs Large Language Models (LLMs) to \textit{generate new answers} that \textit{approximate} these ideal counterfactuals. We denote these LLM-generated approximations as $\tilde{\mathrm{A}}^{(\cdot)}$. For instance, $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{degraded})}$ is an LLM rewrite of $\mathrm{A}$ that attempts to specifically degrade its quality along the causal attribute $C_j$, with explicit instructions to make "minimal changes" and preserve other attributes as much as possible.

% \begin{remark}
% It is crucial to note that in \carma{}, causal attributes $\mathrm{C}(\mathrm{A})$ and spurious attributes $\mathrm{SP}(\mathrm{A})$ are first identified or inferred \textit{from an existing answer} $\mathrm{A}$. The generation of an approximated counterfactual answer $\tilde{\mathrm{A}}^{(\cdot)}$ is a subsequent step. This new answer $\tilde{\mathrm{A}}^{(\cdot)}$ is constructed by an LLM with the goal of embodying a specific change (e.g., $C_j \leftarrow \text{degraded}$) relative to the original $\mathrm{A}$, while attempting to hold other attributes constant. This process creates a \textit{new textual instance} whose attributes approximate the desired counterfactual state. While perfect isolation is challenging and these are approximations, they provide a valuable training signal for disentangling attribute contributions to the reward.
% \end{remark}

% {\color{blue} KS: Being pedantic, but can someone propagate $\tilde{A}_{C \leftarrow c}$ everywhere. This is just standard convention. So better to simply use the subscript.}

\vspace{-0.1in}
\subsection{Augmented Training Data for Causal Disentanglement}
\label{subsec:data_augmentation}

\vspace{-0.1in}
We augment the original preference dataset $\mathcal{D}_{\mathrm{pref}}$ with synthetically generated examples $\mathcal{D}_{\mathrm{aug}}$ designed to enforce specific causal properties on $\hat{\mathrm{R}}_\theta$. This augmented dataset $\mathcal{D}_{\mathrm{aug}}$ comprises two principal categories: Causal Augmentation Pairs ($\mathcal{D}_{\mathrm{causal}}$) and Neutral Augmentation Pairs ($\mathcal{D}_{\mathrm{neutral}}$), summarized in Table \ref{tab:augmentation_summary}.



\vspace{-0.15in}
\begin{table}[!t]
\centering
\caption{Summary of \carma{}'s Synthetic Data Augmentation Strategies using LLM-approximated counterfactuals. $\tilde{\mathrm{A}}^{(C_j \leftarrow target)}$ denotes an LLM rewrite of an original answer $\mathrm{A}$ to set its $j$-th causal attribute $C_j$ to the $target$ state (e.g., "upgraded", "degraded"). 
$\tilde{\mathrm{A}}_{k}^{(C \leftarrow C(A_m))}$ denotes rewriting answer $A_k$ to match the causal attribute profile $C(A_m)$ of answer $A_m$, while aiming to preserve the spurious attributes $SP(A_k)$ of the original $A_k$.}
\label{tab:augmentation_summary}
\vspace{1em}
\newcolumntype{L}{>{\raggedright\arraybackslash}p{2.5cm}} % Column for "Strategy"
\newcolumntype{P}{>{\raggedright\arraybackslash}p{4.5cm}} % Column for "Generation Pair Example"
\newcolumntype{C}{>{\centering\arraybackslash}p{1.3cm}}  % Column for "Assigned Label"
\newcolumntype{R}{>{\raggedleft\arraybackslash}p{2.2cm}}   % Column for "Training Objective (P_theta)"
\begin{tabular}{@{}l L P C R@{}}
\toprule
\textbf{Category} & \textbf{Strategy} & \textbf{Generation Pair Example} & \textbf{Assigned Label} & \textbf{Training Objective ($\mathrm{P}_\theta$)} \\
\midrule
\multicolumn{5}{l}{\textit{Causal Augmentation ($\mathcal{D}_{\mathrm{causal}}$) - Enhancing Sensitivity to $\mathrm{C}$}} \\
\midrule
Causal & Attribute Upgradation/Degradation & $(\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})}, \mathrm{A})$ \textbf{or} $(\mathrm{A}, \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})})$ \newline  & $\succ$ & $\to 1$ \\
% Causal & Attribute Degradation & $(\mathrm{A}, \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})})$ \newline \footnotesize{where $\mathrm{A}$ was good on $C_j$} & $\succ$ & $\to 1$ \\
\midrule
\multicolumn{5}{l}{\textit{Neutral Augmentation ($\mathcal{D}_{\mathrm{neutral}}$) - Enforcing Invariance to $\mathrm{SP}$}} \\
\midrule
Neutral & Irrelevant Pair Comparison (via Query Change) & $(\mathrm{B}_1, \mathrm{B}_2)$ with new $\mathrm{Q}_{\text{irrelevant}}$ \newline \footnotesize{s.t. $\mathrm{C(B_1|Q_{\text{irrelevant}})} \approx \mathrm{C(B_2|Q_{\text{irrelevant}})} \approx \mathbf{0}$} & $ \approx $ (tie) & $\approx 0.5$ \\
\bottomrule
\end{tabular}
\end{table}

% \vspace{-0.05in}



\subsubsection{Causal Augmentation Pairs (\texorpdfstring{$\mathcal{D}_{\mathrm{causal}}$}{D-causal})}
\carma{}'s strategy causal pairs focuses on isolating the impact of important causal attributes.

\vspace{-0.05in}
% \paragraph{1. Attribute Upgradation.} For an original answer $\mathrm{A}$ (typically a lower-quality response $\mathrm{y}_l^{(i)}$ from $\mathcal{D}_{\mathrm{pref}}$ considered poor on a specific causal attribute $\mathrm{C}_j$), we generate an LLM-approximated counterfactual $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{upgraded})}$ where $C_j$ is improved. The pair $(\tilde{\mathrm{A}}^{(C_j \leftarrow \text{upgraded})}, \mathrm{A})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with the label $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{upgraded})} \succ \mathrm{A}$.

\begin{wrapfigure}{r}{0.4\linewidth}
    \centering
    \vspace{-0.1in}
    \includegraphics[width=1.0\linewidth]{images/CausalPerturbations.pdf}
    \vspace{-0.2in}
    \caption{Key \carma{} augmentation examples.
(\textbf{Top}) \textit{Causal Augmentation (Attribute Isolation):} LLM-generated counterfactual $\mathrm{A}'$ isolates a change in a causal attribute $\mathrm{C}(\mathrm{A}|\mathrm{Q})$ of answer $\mathrm{A}$ for query $\mathrm{Q}$, teaching causal sensitivity.
(\textbf{Bottom}) \textit{Neutral Augmentation (Irrelevant Pair Comparison):} Answers $\mathrm{A}$ and $\mathrm{A}'$ (for query $\mathrm{Q}_1$) are both irrelevant to query $\mathrm{Q}_2$, teaching invariance for irrelevant content.\vspace{-0.9in}}
    \label{fig:augmentation_strategies_detail}
\end{wrapfigure}

\paragraph{1. Attribute Isolation via Intervention.}
For an original answer $\mathrm{A}$ (from $\mathcal{D}_{\mathrm{pref}}$) and a specific causal attribute $\mathrm{C}_j$, we generate LLM-approximated counterfactuals.
If $\mathrm{A}$ is of lower quality regarding $\mathrm{C}_j$, we create an upgraded version $\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{upgraded})}$. The pair $(\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{upgraded})}, \mathrm{A})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with label $\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{upgraded})} \succ \mathrm{A}$ post-verification.
Conversely, if $\mathrm{A}$ is of higher quality on $\mathrm{C}_j$, we generate a degraded version $\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{degraded})}$. The pair $(\mathrm{A}, \tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{degraded})})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with label $\mathrm{A} \succ \tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{degraded})}$.
These pairs collectively teach $\hat{\mathrm{R}}_\theta$ sensitivity to changes along individual causal dimensions.


% \paragraph{1. Attribute Upgradation.} From a lower-quality answer $\mathrm{A}$ (from $\mathcal{D}_{\mathrm{pref}}$, poor on causal attribute $C_j$), we generate $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})}$ where $C_j$ is improved. The pair $(\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})}, \mathrm{A})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with label $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})} \succ \mathrm{A}$, after verification that the causal attribute is indeed improved.




% \vspace{-0.05in}
% \paragraph{2. Attribute Degradation.} Conversely, for an original answer $\mathrm{A}$ (typically a higher-quality response $\mathrm{y}_w^{(i)}$ from $\mathcal{D}_{\mathrm{pref}}$ considered good on $C_j$), we create its approximated degraded version $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})}$. The pair $(\mathrm{A}, \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with the label $\mathrm{A} \succ \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})}$.
% Collectively, these teach $\hat{\mathrm{R}}_\theta$ to assign higher scores to improvements along specific causal dimensions.

\subsubsection{Neutral Augmentation Pairs (\texorpdfstring{$\mathcal{D}_{\mathrm{neutral}}$}{D-neutral})}
These pairs (assigned tie-labels) teach invariance to $\mathrm{SP}(\mathrm{A})$ when $\mathrm{C}(\mathrm{A})$ is held constant or is irrelevant.


% \vspace{-0.1in}
% Given an original preference pair $(\mathrm{A}_1, \mathrm{A}_2)$ from $\mathcal{D}_{\mathrm{pref}}$ (e.g., $\mathrm{A}_1 \succ \mathrm{A}_2$), we prompt an LLM to rewrite $\mathrm{A}_2$ to match the causal attributes of $\mathrm{A}_1$ while attempting to retain the spurious characteristics of $\mathrm{A}_2$, yielding $\tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))}$. The pair $(\mathrm{A}_1, \tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))})$ is labeled as a tie. This strategy is often applied in direct conjunction with original preference data or outputs of causal augmentation, ensuring invariance is learned over relevant attribute distributions.
% \paragraph{1. Causally-Aligned Reconstruction.}
% Given an original preference pair $(\mathrm{A}_1, \mathrm{A}_2)$ (e.g., $\mathrm{A}_1 \succ \mathrm{A}_2$), an LLM rewrites $\mathrm{A}_2$ to match $C(A_1)$ while attempting to retain $SP(A_2)$, yielding $\tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))}$. The pair $(\mathrm{A}_1, \tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))})$ is labeled as a tie. 
% $A_1$ and $\tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))}$ are now (approximately) causally equivalent but differ in their spurious attributes via $SP(A_1)$ vs. $SP(\tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))})$, which is influenced by $SP(A_2)$ as well as confounders $U$ in the new generative process. This effectively enforces invariance learning along these specific spurious variations ($SP(\cdot)$) when causal content is aligned.




% Such an $\tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))}$ is generated through a new model (with different $U$) from the original $A_2$ generator, hence we expect that $SP(A_2) \neq SP(\tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))})$.
% This enforces invariance learning over the spurious features $SP(\cdot)$.

% This enforces invariance learning over the spurious features $SP(\cdot)$.
% This is often applied in conjunction with original or causally manipulated data, ensuring invariance is learned over relevant attribute distributions.


\vspace{-0.1in} % Keep if needed
\paragraph{Irrelevant Pair Comparison (via Query Modification).}
We pair two answers, $\mathrm{B}_1, \mathrm{B}_2$ (often from $\mathcal{D}_{\mathrm{causal}}$, e.g., $\mathrm{A}$ and $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{target})}$), with a \textit{new, unrelated query} $\mathrm{Q}_{\text{irrelevant}}$. This makes their causal attributes w.r.t. $\mathrm{Q}_{\text{irrelevant}}$ (i.e., $\mathrm{C(B_1|Q_{\text{irrelevant}})}, \mathrm{C(B_2|Q_{\text{irrelevant}})}$) minimal. The pair $(\mathrm{B}_1, \mathrm{B}_2)$ under $\mathrm{Q}_{\text{irrelevant}}$ receives a tie-label, training the RM to disregard spurious differences when causal relevance is absent. Their original causal distinction for their original query becomes moot, isolating spurious variations under $\mathrm{Q}_{\text{irrelevant}}$.

% \vspace{-0.1in}
% \paragraph{2. Irrelevant Pair Comparison (via Query Modification).}
% Given two answers $\mathrm{B}_1, \mathrm{B}_2$, we pair them with a new, unrelated query $\mathrm{Q}_{\text{new}}$. Relative to $\mathrm{Q}_{\text{new}}$, both $C(B_1|\mathrm{Q}_{\text{new}})$ and $C(B_2|\mathrm{Q}_{\text{new}})$ become effectively zero (i.e., causally irrelevant). The pair $(\mathrm{B}_1, \mathrm{B}_2)$ for query $\mathrm{Q}_{\text{new}}$ is then labeled as a tie, teaching invariance when causal quality is uniformly low, regardless of variations in spurious features. Concretely, let us say efficiency was a relevant (causal) feature for a coding related question, by swapping out the query, efficiency may become irrelevant. Due to this reason we find (as shown in Section \ref{subsec:experimental_results}) that irrelevant pair comparison is more powerful when done on causal pairs,  since causal pairs differ on only one attribute, which is likely to be irrelevant for a random swapped question. 



\vspace{-0.05in}
Further details on these generation strategies, their relationship with other methods (like Relevance Contrast or direct Spurious Perturbation), and the rationale for \carma{}'s specific choices are discussed in Appendix \ref{sec:causal_model_details}. 
% The combined dataset $\mathcal{D} = \mathcal{D}_{\mathrm{pref}} \cup \mathcal{D}_{\mathrm{causal}} \cup \mathcal{D}_{\mathrm{neutral}}$ (after filtering imperfect augmentations, see Section \ref{subsec:filtering_appendix}) provides the signal for robust training. The central idea is that explicit examples of disentanglement are key to teaching a reward model to distinguish causal quality drivers from spurious correlates. 
We provide the prompts for the generations described in Section \ref{sec:prompt_templates}.

==> archived/np_20250611.tex <==

\vspace{-0.1in}
\section{Causal Framework for Reward Modeling}
\label{sec:preliminaries}

\vspace{-0.05in}
% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{images/causalDiagram.pdf} 
% \caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query, $\mathcal{I}$ is the latent intent for the response, $\mathcal{U}$ is the set of unknown confounders from the generator, $\mathrm{A}$ is the generated answer, $\mathrm{C}(\mathrm{A})$ are causal attributes, $\mathrm{SP}(\mathrm{A})$ are spurious attributes, and $\mathrm{R}^*$ is the ground-truth reward. The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, such that its dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$.}
% \label{fig:causal_graph}
% \end{figure}

% \vspace{-0.1in}
% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.7\linewidth]{images/CausalGraphA.pdf} 
% \caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query. The Answer (A) comprises of two types of attributes, $\mathrm{C}(\mathrm{A})$, which are causal attributes, and $\mathrm{SP}(\mathrm{A})$ which are spurious attributes. $\mathrm{R}^*$ is the human annotated or ground-truth reward which are posited to depend only on C(A). The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, such that its dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$. \vspace{-0.2in}}
% \label{fig:causal_graph}
% \end{figure}


\begin{figure}[!t]               % one float, two columns inside
  \centering
  \begin{minipage}[t]{0.58\textwidth}
    \vspace{0.0in}
    \centering
    \includegraphics[width=\linewidth]{images/CausalGraphA.pdf}
    % \vspace{-0.1in}
    % \captionof{figure}{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query. Answer (A) has causal attributes $\mathrm{C}(\mathrm{A})$ and spurious attributes $\mathrm{SP}(\mathrm{A})$. Ground-truth reward $\mathrm{R}^*$ depends only on $\mathrm{C(A)}$ and $\mathrm{Q}$. Augmentations heighten $\hat{\mathrm{R}}_\theta$'s sensitivity to $\mathrm{C(A)}$ (approximated by oracle LLM).}
    
  \end{minipage}\hfill
  \begin{minipage}[t]{0.4\textwidth}
        \centering
        \vspace{-0.25in}
        \resizebox{\linewidth}{!}{% Make table fit the minipage width
        \begin{tabular}{c|p{0.75\linewidth}} % Adjusted width for p column, assuming overall table width constraint
\toprule
\textbf{Path/ Relationship} & \textbf{Interpretation Summary} \\
\midrule
$(\mathrm{Q}, \mathrm{C}(\mathrm{A})) \to \mathrm{R}^*$ & Ground-truth reward $\mathrm{R}^*$ determined by query $\mathrm{Q}$ and causal attributes $\mathrm{C(A)}$; stable relationship. \\
$\mathrm{Q} \leftrightarrow \mathrm{SP(A)}$  & Query $\mathrm{Q}$ and unknown spurious attributes $\mathrm{SP(A)}$ are correlated/confounded by unstable exogenous factors. \\
$\mathrm{Q} \to \mathrm{C(A)}$ & Query $\mathrm{Q}$ determines relevant causal attributes $\mathrm{C(A)}$. \\
$\mathrm{SP(A)} \leftrightarrow \mathrm{C(A)}$ & Bidirectional (potentially complex) relationship between spurious $\mathrm{SP(A)}$ and causal $\mathrm{C(A)}$ attributes. \\
\bottomrule
\end{tabular}
        } % End resizebox
        % \vspace{-0.1in}
        % \caption{$\mathrm{R^*} \perp \mathrm{SP(A)} | \mathrm{C(A)}$, Q. $\text{dim}(C(A)) \gg \text{dim}(SP(A)) \forall A$. $\mathrm{SP(A)}$ is unknown. \vspace{-0.2in}}
        \label{tab:causal_arrows}
  \end{minipage}\hfill          % \hfill inserts a flexible gutter
  % \vspace{-0.2in}
\caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query. Answer (A) has causal attributes $\mathrm{C}(\mathrm{A})$ and spurious attributes $\mathrm{SP}(\mathrm{A})$. $\text{dim}(C(A)) \ll \text{dim}(SP(A))\ \forall A$. $\mathrm{SP(A)}$ is unknown. Ground-truth reward $\mathrm{R}^*$ depends only on $\mathrm{C(A)}$ and $\mathrm{Q}$ ($\mathrm{R^*} \perp \mathrm{SP(A)} | \mathrm{C(A)}$, Q). Augmentations heighten $\hat{\mathrm{R}}_\theta$'s sensitivity to $\mathrm{C(A)}$ (approximated by oracle LLM).}
\label{fig:causal_graph}
\vspace{-0.15in}
\end{figure}
  % \vspace{0.03in}


% \vspace{-0.1in}
% \begin{figure}[t!]
% \centering
% \includegraphics[width=\linewidth]{images/CausalGraphNew.pdf} 
% \caption{Conceptual Causal Graph for Reward Modeling. $\mathrm{Q}$ is the query, $\mathcal{I}$ is the latent intent for the response, $\mathcal{U}$ is the set of unknown confounders from the generator, $\mathrm{A}$ is the generated answer, $\mathrm{C}(\mathrm{A})$ are causal attributes, $\mathrm{SP}(\mathrm{A})$ are spurious attributes, and $\mathrm{R}^*$ is the ground-truth reward. The goal is to train $\hat{\mathrm{R}}_\theta$ to estimate $\mathrm{R}^*$, such that its dependence on $\mathrm{A}$ is primarily mediated through $\mathrm{C}(\mathrm{A})$.}
% \label{fig:causal_graph}
% \end{figure}

\vspace{-0.05in}
We aim to develop a reward model that accurately assesses the quality of an answer $\mathrm{A}$ provided in response to a query $\mathrm{Q}$. Our approach is grounded in a causal framework designed to distinguish genuine quality drivers from spurious correlates often present in preference data. This involves understanding the answer generation process and strategically augmenting training data with approximated counterfactual examples.

\vspace{-0.1in}
\subsection{Reward Model and Pairwise Preferences}
We train a reward model (RM), denoted $\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A})$, to assign a scalar quality score to an answer $\mathrm{A}$ for a query $\mathrm{Q}$. This RM is typically optimized on a dataset  preferences pairs $\mathcal{D}_{\mathrm{pref}} = \{(\mathrm{Q}^{(i)}, \mathrm{y}_w^{(i)}, \mathrm{y}_l^{(i)})\}_{i=1}^N$. Given a pair of answers $(\mathrm{A}_1, \mathrm{A}_2)$, the probability of $\mathrm{A}_1$ being preferred over $\mathrm{A}_2$ is commonly modeled using the Bradley-Terry framework \citep{bradley1952rank}:
\begin{equation}
\mathrm{P}(\mathrm{A}_1 \succ \mathrm{A}_2 | \mathrm{Q}; \theta) = \sigmoid(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{s}_\theta(\mathrm{Q}, \mathrm{A}_2)) = \frac{\exp(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1))}{\exp(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1)) + \exp(\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_2))}
\label{eq:bt_prob_roman}
\end{equation}
where $\hat{s}_\theta(\mathrm{Q}, \mathrm{A})$ represents the underlying scalar score (or logit) assigned by the model to answer $\mathrm{A}$ for query $\mathrm{Q}$. \footnote{The score $\hat{s}_\theta(\mathrm{Q}, \mathrm{A})$ can be the direct output of a reward head or, in some pairwise preference models, $\hat{s}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{s}_\theta(\mathrm{Q}, \mathrm{A}_2)$ might be directly modeled as the logit of preferring $\mathrm{A}_1$ over $\mathrm{A}_2$.} The parameters $\theta$ are learned by minimizing the negative log-likelihood of  preferences.

% \subsection{Reward Model and Pairwise Preferences}
% Let $\hat{\mathrm{R}}(\mathrm{Q}, \mathrm{A})$ denote the learned reward model, which assigns a scalar score reflecting the quality of answer $\mathrm{A}$ for query $\mathrm{Q}$. While $\hat{\mathrm{R}}$ provides a pointwise score, it is typically trained using pairwise preference data. Given two answers $\mathrm{A}_1$ and $\mathrm{A}_2$ for the same query $\mathrm{Q}$, we relate the reward scores to preference probabilities using the Bradley-Terry model \citep{bradley1952rank}:
% \begin{equation}
% \mathrm{P}(\mathrm{A}_1 \succ \mathrm{A}_2 | \mathrm{Q}; \theta) = \sigmoid(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1) - \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2)) = \frac{\exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1))}{\exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_1)) + \exp(\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_2))}
% \label{eq:bt_prob_roman}
% \end{equation}
% where $\hat{\mathrm{R}}_\theta$ explicitly denotes the model parameterized by $\theta$, and $\sigmoid(\cdot)$ is the logistic sigmoid function. The parameters $\theta$ are optimized using a dataset of observed preferences $\mathcal{D}_{\mathrm{pref}} = \{(\mathrm{Q}^{(i)}, \mathrm{y}_w^{(i)}, \mathrm{y}_l^{(i)})\}_{i=1}^N$, typically by minimizing the negative log-likelihood based on Eq. \ref{eq:bt_prob_roman}.


% \vspace{-0.15in}
\begin{table}[!t]
\centering
% \caption{Summary of \carma{}'s Synthetic Data Augmentation Strategies using LLM-approximated counterfactuals. $\tilde{\mathrm{A}}^{(C_j \leftarrow target)}$ denotes an LLM rewrite of an original answer $\mathrm{A}$ to set its $j$-th causal attribute $C_j$ to the $target$ state (e.g., "upgraded", "degraded"). 
% $\tilde{\mathrm{A}}_{k}^{(C \leftarrow C(A_m))}$ denotes rewriting answer $A_k$ to match the causal attribute profile $C(A_m)$ of answer $A_m$, while aiming to preserve the spurious attributes $SP(A_k)$ of the original $A_k$.}
\vspace{-0.1in}
\vspace{1em}
\newcolumntype{L}{>{\raggedright\arraybackslash}p{5.0cm}} % Column for "Strategy"
\newcolumntype{P}{>{\raggedright\arraybackslash}p{5.0cm}} % Column for "Generation Pair Example"
\newcolumntype{C}{>{\centering\arraybackslash}p{1.3cm}}  % Column for "Assigned Label"
\newcolumntype{R}{>{\raggedleft\arraybackslash}p{2.5cm}}   % Column for "Training Objective (P_theta)"
\begin{tabular}{@{}l L P C R@{}}
\toprule
\textbf{Category} & \textbf{Strategy} & \textbf{Generation Pair Example} & \textbf{Assigned Label} & \textbf{Training Objective ($\mathrm{P}_\theta$)} \\
\midrule
\multicolumn{5}{l}{\textit{Causal Augmentation} ($\mathcal{D}_{\mathrm{causal}}$) - Enhancing Sensitivity to $\mathrm{C}$} \\
\midrule
Causal & Attribute Upgradation/Degradation & $(\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})}, \mathrm{A})$ \textbf{or} $(\mathrm{A}, \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})})$ \newline  & $\succ$ & $\to 1$ \\
% Causal & Attribute Degradation & $(\mathrm{A}, \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})})$ \newline \footnotesize{where $\mathrm{A}$ was good on $C_j$} & $\succ$ & $\to 1$ \\
\midrule
\multicolumn{5}{l}{\textit{Neutral Augmentation} ($\mathcal{D}_{\mathrm{neutral}}$) - \textit{Enforcing Invariance to} $\mathrm{SP}$} \\
\midrule
Neutral & Irrelevant Pair Comparison (via Query Change) & $(\mathrm{B}_1, \mathrm{B}_2)$ with irrelevant $\mathrm{Q}_{\text{irrelevant}}$ \newline \footnotesize{s.t. $\mathrm{C(B_1|Q_{\text{irrelevant}})} \approx \mathrm{C(B_2|Q_{\text{irrelevant}})} \approx \mathbf{0}$} & $ \approx $ (tie) & $\approx 0.5$ \\
\bottomrule
\end{tabular}
\caption{Summary of \carma{}'s synthetic data augmentation strategies using LLM-approximated counterfactuals. $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{target})}$ signifies an LLM-generated counterfactual of $\mathrm{A}$ with its $j$-th causal attribute $C_j$ modified.}
\label{tab:augmentation_summary}
\vspace{-0.15in}
\end{table}

\vspace{-0.05in}
\subsection{A Causal Model of Answer Generation}
\label{subsec:causal_graph}

\vspace{-0.05in}
We propose a causal model (Figure \ref{fig:causal_graph}) for answer generation and quality perception. For a query-answer pair $(\mathrm{Q}, \mathrm{A})$, we distinguish two attribute types:

\vspace{-0.1in}
\begin{itemize}[itemsep=0pt,left=0pt]
    \item \textbf{Causal Attributes} $\mathrm{C}(\mathrm{A}) = \{\mathrm{C}_1, \dots, \mathrm{C}_\ell\}$: Fundamental quality dimensions (e.g., factuality, relevance) genuinely determining quality relative to $\mathrm{Q}$.
    \item \textbf{Spurious Attributes} $\mathrm{SP}(\mathrm{A}) = \{\mathrm{SP}_1, \dots, \mathrm{SP}_k\}$: Other features (e.g., length, formatting) correlated with preferences or $\mathrm{Q}$ in $\mathcal{D}_{\mathrm{pref}}$, but not intrinsically determining quality. $\mathrm{SP}(\mathrm{A})$ can be high-dimensional and unknown.
\end{itemize}

\vspace{-0.1in}
The ground-truth reward $\mathrm{R}^*(\mathrm{Q}, \mathrm{A})$ is assumed to be solely a function of causal attributes: $\mathrm{R}^*(\mathrm{Q}, \mathrm{A}) = f^*(\mathrm{Q}, \mathrm{C}(\mathrm{A}))$. This implies conditional independence: $\mathrm{R}^* \perp \mathrm{SP}(\mathrm{A}) | \mathrm{Q}, \mathrm{C}(\mathrm{A})$.

We explicitly assume the following stability property: \textit{If the entire process of answer generation and reward labeling were repeated (e.g., with a different labeler or answer generator), the relationship $(\mathrm{Q}, \mathrm{C}(\mathrm{A})) \to \mathrm{R}^{*}$ determining the reward is stable/invariant.} In contrast, correlations involving $\mathrm{SP}(\mathrm{A})$ (e.g., $\mathrm{SP}(\mathrm{A}) \leftrightarrow \mathrm{C}(\mathrm{A})$ or $\mathrm{SP}(\mathrm{A}) \leftrightarrow \mathrm{Q}$) can arise from various, potentially unstable or unknown exogenous factors, and thus these correlations may vary across such repetitions.

The primary challenge is that standard reward models $\hat{\mathrm{R}}_\theta$ may inadvertently learn high sensitivity to these unstable correlations with $\mathrm{SP}(\mathrm{A})$ (due to its unknown, high-dimensional nature). Our goal is to train $\hat{\mathrm{R}}_\theta$ such that its dependence on $\mathrm{A}$ is primarily mediated through the identified, stable causal attributes $\mathrm{C}(\mathrm{A})$, ensuring robustness to unspecified $\mathrm{SP}(\mathrm{A})$.

% We propose a causal model (Figure \ref{fig:causal_graph}) to analyze the generation of answers and how their quality is perceived. The process begins with a query, answer pair $\mathrm{Q},\mathrm{A}$ that is rated by a human or some other agent providing ground truth reward label. {\color{blue} The answer has two parts, one being causal attributes ($C(A)$) and the other being spurious attributes ($SP(A)$). The reward labeler (or human) uses causal attributes ($C(A)$) to provide ground truth reward label that is part of the training data. All other features are considered to be $SP(A)$ and are correlated with $C(A)$. Further, at the time of answer generation, there may be unknown factors (additional prompts to condition the answer, or unknown exogenous confounding factors) that correlate spurious factors $SP(A)$ with the question. 
% We assume the following: \textit{If the entire process is repeated with different labeler and answer generator, then $Q, C(A) \rightarrow R^{*}$ relationship of reward labeling  is stable/invariant compared to unstable correlation between spurious factors and the question.}}




% \begin{table}[t!]
% \centering
% \caption{Explanation of the Causal Model}
% \label{tab:causal_arrows}
% \vspace{1em}
% \begin{tabular}{c|p{9cm}} % Adjusted widths
% \toprule
% \textbf{Arrow} & \textbf{Interpretation} \\
% \midrule
% $(\mathrm{Q}, \mathrm{C}(\mathrm{A})) \;\to\; \mathrm{R}^*$ & The ground-truth reward $\mathrm{R}^*$ is solely determined by the causal attributes $\mathrm{C(A)}$ and the question $\mathrm{Q}$. The labeling agent is looks  at only $\mathrm{C(A)}$ and $\mathrm{Q}$ to decide on the label. This relationships is assumed to be stable across labeling agents. \\
% $\mathrm{Q}\leftrightarrow \mathrm{SP(A)}$  & $\mathrm{SP(A)}$ - all unknown spurious attributes that is not $\mathrm{C(A)}$ but correlated/confounded with question through unknown factors. This correlation is unstable and is different depending on other exogenous factors.  \\
% $\mathrm{Q}\rightarrow \mathrm{C(A)}$ & Question determines causal attributes of the answer relevant to the reward \\
% $\mathrm{SP(A)} \leftrightarrow \mathrm{C(A)}$ & Causal and spurious attributes have bidirectional relationship. Specifically we will model $SP_1(A) \subseteq SP(A)$ that has no parents in $C(A)$, and $SP_2(A) \subset SP(A)$ with direct parents in $C(A)$ \\

% %$\mathrm{A} \;\to\; \mathrm{C}(\mathrm{A})$ & The answer text manifests causal quality attributes. \\
% %$\mathrm{A} \;\to\; \mathrm{SP}(\mathrm{A})$ & The answer text also manifests spurious attributes. \\
% \midrule
% \multicolumn{2}{p{12cm}}{\textbf{Note:} Key property is the conditional independence $\mathrm{R^*} \perp \mathrm{SP(A)} | \mathrm{C(A)}$. $\mathrm{SP(A)}$ is unknown and potentially very high dimensional ($k >> \ell$). Our augmentation strategies are aimed at heightening sensitivity of reward to $\mathrm{C(A)}$ by varying answers along these only. An approximation to $\mathrm{C(A)}$ is obtained by querying an oracle LLM.  } \\
% \bottomrule
% \end{tabular}
% \end{table} 



\vspace{-0.1in}
\subsection{Approximating Counterfactuals for Attribute Intervention}
\label{subsec:approximating_counterfactuals}
\vspace{-0.05in}

To instill causal sensitivity and spurious invariance in $\hat{\mathrm{R}}_\theta$, \carma{} leverages counterfactual reasoning about how answer quality changes if specific attributes were altered. For an answer $\mathrm{A}$ with attributes $(\mathrm{C}(\mathrm{A}), \mathrm{SP}(\mathrm{A}))$, an ideal counterfactual, $A_{(C_j \leftarrow c'_j)}(u)$, would manifest if only its $j$-th causal attribute $C_j$ were set to $c'_j$, considering its causal effects on other features, while all other exogenous factors $u$ (that produced the factual answer $a$) remained constant. Formally, $P_{U}(A_{(C_j \leftarrow c'_j)}(U) | A(U)=a)$.
% {\color{brown}GP: It would be nice to explain (more clearly) on how the notation should be interpreted. It is not clear at the moment. A few minor issues e.g. the explanation for what ``u'' means comes much later after the variable is introduced.}

As generating such ideal textual counterfactuals is intractable, \carma{} employs Large Language Models (LLMs) to produce \textit{approximations}. These LLM-generated answers, denoted $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{target})}$, are rewrites of an original answer $\mathrm{A}$, prompted to modify $C_j$ (e.g., to a "degraded" state, lowering reward) while aiming for minimal changes to other attributes.



\begin{remark}
For brevity, we denote these LLM approximations as $\tilde{\mathrm{A}}_{(C_j \leftarrow c)}$, dropping the explicit $u$ conditioning, assuming the generation approximates such a sample. While imperfect, these approximations provide the targeted variations crucial for our data augmentation.
\end{remark}

% \vspace{-0.05in}
% \subsection{Construction of Counterfactuals when causal attributes change}
% \label{subsec:approximating_counterfactuals}

% \vspace{-0.05in}
% {\color{blue}
% To train $\hat{\mathrm{R}}_\theta$ for causal sensitivity and spurious invariance, we leverage the concept of counterfactuals: reasoning about how an answer's quality would change if specific attributes were altered. Given an answer $\mathrm{A}$ with attributes $(\mathrm{C}(\mathrm{A}), \mathrm{SP}(\mathrm{A}))$, an ideal counterfactual $A_{(C_j \leftarrow c'_j)} (u)$ would represent $\mathrm{A}$ with only its $j$-th causal attribute $C_j$ changed to $c'_j$ and its effect on other features through their causal relationships, given all else (all hidden factors of variation captured in variable $u$) held in those values that would give rise to the factual answer. Formally, the counterfactual is sampled from $P_{U}(A_{(C_j \leftarrow c'_j)} (U) | A(U) =a)$ - a counterfactual distribution under the exogenous conditional distribution $u$ that gives rise to the factual answer $a$ and under the intervention $(C_j \leftarrow c'_j)$.

% Perfectly constructing such ideal textual counterfactuals is intractable. \carma{} therefore employs Large Language Models (LLMs) to \textit{generate new answers}, denoted $\tilde{\mathrm{A}}_{(\cdot)}$, that \textit{approximate} these ideal counterfactuals. For example, $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})}(u)$ is an LLM rewrite of the original answer $\mathrm{A}$, prompted to degrade $C_j$, in the sense of lowering the reward, while minimally affecting other attributes. }

% {\color{blue}
% \begin{remark} For the sake of brevity in what follows, we use $\tilde{A}_{C_j \leftarrow c}$ dropping the dependence on exogenous condition $u$ sampled under condition $A(u) = a$. We assume that the generated answer approximately reflects such a sample. While these are approximations and perfect attribute isolation is difficult, they provide the targeted variations necessary for our data augmentation.
% \end{remark}
% }
% \begin{remark}
% In \carma{}, attributes are identified from an existing answer $\mathrm{A}$. An LLM then constructs a \textit{new textual instance} $\tilde{\mathrm{A}}^{(\cdot)}$ to approximate a desired counterfactual state (e.g., $C_j$ modified). 
% \end{remark}

% \subsection{Approximating Counterfactual Answer Variations}
% \label{subsec:approximating_counterfactuals}

% To teach $\hat{\mathrm{R}}_\theta$ the desired sensitivities and invariances, we reason about \textit{counterfactual answers}: what an answer \textit{would have been like} if certain attributes had been different. Given an original answer $\mathrm{A}$ (with its observed attributes $\mathrm{C}(\mathrm{A})$ and $\mathrm{SP}(\mathrm{A})$), we consider an ideal counterfactual, such as $A^{(C_j \leftarrow c'_j)}$, where only the $j$-th causal attribute $C_j$ is hypothetically changed to $c'_j$, while all other causal attributes $\mathrm{C}_{k \neq j}(\mathrm{A})$ and all spurious attributes $\mathrm{SP}(\mathrm{A})$ are held constant.

% Directly constructing such ideal counterfactual answers from a given text $\mathrm{A}$ while perfectly isolating attribute changes is generally intractable. \carma{} employs Large Language Models (LLMs) to \textit{generate new answers} that \textit{approximate} these ideal counterfactuals. We denote these LLM-generated approximations as $\tilde{\mathrm{A}}^{(\cdot)}$. For instance, $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{degraded})}$ is an LLM rewrite of $\mathrm{A}$ that attempts to specifically degrade its quality along the causal attribute $C_j$, with explicit instructions to make "minimal changes" and preserve other attributes as much as possible.

% \begin{remark}
% It is crucial to note that in \carma{}, causal attributes $\mathrm{C}(\mathrm{A})$ and spurious attributes $\mathrm{SP}(\mathrm{A})$ are first identified or inferred \textit{from an existing answer} $\mathrm{A}$. The generation of an approximated counterfactual answer $\tilde{\mathrm{A}}^{(\cdot)}$ is a subsequent step. This new answer $\tilde{\mathrm{A}}^{(\cdot)}$ is constructed by an LLM with the goal of embodying a specific change (e.g., $C_j \leftarrow \text{degraded}$) relative to the original $\mathrm{A}$, while attempting to hold other attributes constant. This process creates a \textit{new textual instance} whose attributes approximate the desired counterfactual state. While perfect isolation is challenging and these are approximations, they provide a valuable training signal for disentangling attribute contributions to the reward.
% \end{remark}

% {\color{blue} KS: Being pedantic, but can someone propagate $\tilde{A}_{C \leftarrow c}$ everywhere. This is just standard convention. So better to simply use the subscript.}

\vspace{-0.1in}
\subsection{Augmented Training Data for Causal Disentanglement}
\label{subsec:data_augmentation}


\vspace{-0.1in}
We augment the original preference dataset $\mathcal{D}_{\mathrm{pref}}$ with synthetically generated examples $\mathcal{D}_{\mathrm{aug}}$ designed to enforce specific causal properties on $\hat{\mathrm{R}}_\theta$. This augmented dataset $\mathcal{D}_{\mathrm{aug}}$ comprises two principal categories: Causal Augmentation Pairs ($\mathcal{D}_{\mathrm{causal}}$) and Neutral Augmentation Pairs ($\mathcal{D}_{\mathrm{neutral}}$), summarized in Table \ref{tab:augmentation_summary}.


\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{images/CausalAugmentationProcess_Horizontal.pdf}
  \vspace{-0.2in}
%   \caption{\textbf({Top}) \textit{Causal Augmentation:} LLM-generated counterfactual $\mathrm{A2}$ isolates a change in a causal attribute $\mathrm{C}(\mathrm{A1}|\mathrm{Q})$ of answer $\mathrm{A1}$ for query $\mathrm{Q}$, teaching causal sensitivity.
% ({Bottom}) \textit{Neutral Augmentation:} Answers $\mathrm{A1}$ and $\mathrm{A2}$ are both irrelevant to query $\mathrm{Q}_{new}$, teaching invariance for irrelevant content.}
%   \label{fig:augmentation_strategies_detail}
  \caption{Visualizing \carma's core augmentation strategies (detailed in Appendix~\ref{app:detailed_augmentation_diagrams}).
\textbf{(Top) Causal Augmentation:} For a given query, we use an LLM-driven counterfactual generation process to alter a specific causal attribute, yielding Answer 2. Some spurious attributes may co-vary. The RM is trained with a preference (e.g., $A_1 \succ A_2$ if $A_2$ is a degradation), teaching causal sensitivity.
\textbf{(Bottom) Irrelevant Query Neutral:} The same answer pair ($A_1, A_2$) is re-contextualized with a new, irrelevant question. Their original causal attributes become effectively spurious or irrelevant (greyed-out bar). The RM is trained with a tie-label ($A_1 \approx A_2$), teaching invariance to the  attribute differences when no true causal signal for the current query exists.\vspace{-0.2in}}
\label{fig:carma_augmentation_visual_overview}
  
\end{figure}

% \begin{wrapfigure}{r}{0.6\linewidth}
%     \centering
%     \vspace{-0.5in}
%     \includegraphics[width=1.0\linewidth]{images/CausalPerturbations.pdf}
%     \vspace{-0.25in}
%     \caption{(\textbf{Top}) \textit{Causal Augmentation:} LLM-generated counterfactual $\mathrm{A}'$ isolates a change in a causal attribute $\mathrm{C}(\mathrm{A}|\mathrm{Q})$ of answer $\mathrm{A}$ for query $\mathrm{Q}$, teaching causal sensitivity.
% (\textbf{Bottom}) \textit{Neutral Augmentation:} Answers $\mathrm{A}$ and $\mathrm{A}'$ (for query $\mathrm{Q}_{new}$) are both irrelevant to query $\mathrm{Q}_2$, teaching invariance for irrelevant content.\vspace{-0.9in}}
%     \label{fig:augmentation_strategies_detail}
% \end{wrapfigure}

% \vspace{-0.05in}



\subsubsection{Causal Augmentation Pairs}
\carma{}'s strategy causal pairs $\mathcal{D}_{\mathrm{causal}}$ focus on isolating the impact of important causal attributes.


% \paragraph{1. Attribute Upgradation.} For an original answer $\mathrm{A}$ (typically a lower-quality response $\mathrm{y}_l^{(i)}$ from $\mathcal{D}_{\mathrm{pref}}$ considered poor on a specific causal attribute $\mathrm{C}_j$), we generate an LLM-approximated counterfactual $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{upgraded})}$ where $C_j$ is improved. The pair $(\tilde{\mathrm{A}}^{(C_j \leftarrow \text{upgraded})}, \mathrm{A})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with the label $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{upgraded})} \succ \mathrm{A}$.


\vspace{-0.1in}
\paragraph{Attribute Upgradation and Degradation.}
For an original answer $\mathrm{A}$ (from $\mathcal{D}_{\mathrm{pref}}$) and a specific causal attribute $\mathrm{C}_j$, we generate LLM-approximated counterfactuals.
If $\mathrm{A}$ is of lower quality regarding $\mathrm{C}_j$, we create an upgraded version $\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{upgraded})}$. The pair $(\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{upgraded})}, \mathrm{A})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with label $\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{upgraded})} \succ \mathrm{A}$ post-verification.
Conversely, if $\mathrm{A}$ is of higher quality on $\mathrm{C}_j$, we generate a degraded version $\tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{degraded})}$. The pair $(\mathrm{A}, \tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{degraded})})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with label $\mathrm{A} \succ \tilde{\mathrm{A}}_{(\mathrm{C}_j \leftarrow \text{degraded})}$.
These pairs collectively teach $\hat{\mathrm{R}}_\theta$ sensitivity to changes along individual causal dimensions.


% \paragraph{1. Attribute Upgradation.} From a lower-quality answer $\mathrm{A}$ (from $\mathcal{D}_{\mathrm{pref}}$, poor on causal attribute $C_j$), we generate $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})}$ where $C_j$ is improved. The pair $(\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})}, \mathrm{A})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with label $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{upgraded})} \succ \mathrm{A}$, after verification that the causal attribute is indeed improved.




% \vspace{-0.05in}
% \paragraph{2. Attribute Degradation.} Conversely, for an original answer $\mathrm{A}$ (typically a higher-quality response $\mathrm{y}_w^{(i)}$ from $\mathcal{D}_{\mathrm{pref}}$ considered good on $C_j$), we create its approximated degraded version $\tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})}$. The pair $(\mathrm{A}, \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})})$ is added to $\mathcal{D}_{\mathrm{causal}}$ with the label $\mathrm{A} \succ \tilde{\mathrm{A}}_{(C_j \leftarrow \text{degraded})}$.
% Collectively, these teach $\hat{\mathrm{R}}_\theta$ to assign higher scores to improvements along specific causal dimensions.

\subsubsection{Neutral Augmentation Pairs}
$\mathcal{D}_{\mathrm{neutral}}$ pairs (with tie-labels) teach invariance to $\mathrm{SP}(\mathrm{A})$ when $\mathrm{C}(\mathrm{A})$ is held constant/ is irrelevant.


% \vspace{-0.1in}
% Given an original preference pair $(\mathrm{A}_1, \mathrm{A}_2)$ from $\mathcal{D}_{\mathrm{pref}}$ (e.g., $\mathrm{A}_1 \succ \mathrm{A}_2$), we prompt an LLM to rewrite $\mathrm{A}_2$ to match the causal attributes of $\mathrm{A}_1$ while attempting to retain the spurious characteristics of $\mathrm{A}_2$, yielding $\tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))}$. The pair $(\mathrm{A}_1, \tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))})$ is labeled as a tie. This strategy is often applied in direct conjunction with original preference data or outputs of causal augmentation, ensuring invariance is learned over relevant attribute distributions.
% \paragraph{1. Causally-Aligned Reconstruction.}
% Given an original preference pair $(\mathrm{A}_1, \mathrm{A}_2)$ (e.g., $\mathrm{A}_1 \succ \mathrm{A}_2$), an LLM rewrites $\mathrm{A}_2$ to match $C(A_1)$ while attempting to retain $SP(A_2)$, yielding $\tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))}$. The pair $(\mathrm{A}_1, \tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))})$ is labeled as a tie. 
% $A_1$ and $\tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))}$ are now (approximately) causally equivalent but differ in their spurious attributes via $SP(A_1)$ vs. $SP(\tilde{\mathrm{A}}_{2(C \leftarrow C(A_1))})$, which is influenced by $SP(A_2)$ as well as confounders $U$ in the new generative process. This effectively enforces invariance learning along these specific spurious variations ($SP(\cdot)$) when causal content is aligned.




% Such an $\tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))}$ is generated through a new model (with different $U$) from the original $A_2$ generator, hence we expect that $SP(A_2) \neq SP(\tilde{\mathrm{A}}_{2}^{(C \leftarrow C(A_1))})$.
% This enforces invariance learning over the spurious features $SP(\cdot)$.

% This enforces invariance learning over the spurious features $SP(\cdot)$.
% This is often applied in conjunction with original or causally manipulated data, ensuring invariance is learned over relevant attribute distributions.


\vspace{-0.1in}
\paragraph{Irrelevant Pair Comparison (via Query Modification).}
We pair two answers, $\mathrm{B}_1, \mathrm{B}_2$ (often from $\mathcal{D}_{\mathrm{causal}}$, e.g., $\mathrm{A}$ and $\tilde{\mathrm{A}}^{(C_j \leftarrow \text{target})}$), with a \textit{new, unrelated query} $\mathrm{Q}_{\text{irrelevant}}$. This makes their causal attributes w.r.t. $\mathrm{Q}_{\text{irrelevant}}$ (i.e., $\mathrm{C(B_1|Q_{\text{irrelevant}})}, \mathrm{C(B_2|Q_{\text{irrelevant}})}$) minimal. The pair $(\mathrm{B}_1, \mathrm{B}_2)$ under $\mathrm{Q}_{\text{irrelevant}}$ receives a tie-label, training the RM to disregard spurious differences when causal relevance is absent. Their causal distinction becomes moot, isolating spurious variations under $\mathrm{Q}_{\text{irrelevant}}$.

% \vspace{-0.1in}
% \paragraph{2. Irrelevant Pair Comparison (via Query Modification).}
% Given two answers $\mathrm{B}_1, \mathrm{B}_2$, we pair them with a new, unrelated query $\mathrm{Q}_{\text{new}}$. Relative to $\mathrm{Q}_{\text{new}}$, both $C(B_1|\mathrm{Q}_{\text{new}})$ and $C(B_2|\mathrm{Q}_{\text{new}})$ become effectively zero (i.e., causally irrelevant). The pair $(\mathrm{B}_1, \mathrm{B}_2)$ for query $\mathrm{Q}_{\text{new}}$ is then labeled as a tie, teaching invariance when causal quality is uniformly low, regardless of variations in spurious features. Concretely, let us say efficiency was a relevant (causal) feature for a coding related question, by swapping out the query, efficiency may become irrelevant. Due to this reason we find (as shown in Section \ref{subsec:experimental_results}) that irrelevant pair comparison is more powerful when done on causal pairs,  since causal pairs differ on only one attribute, which is likely to be irrelevant for a random swapped question. 



\vspace{-0.05in}
Further details on these generation strategies, their relationship with other methods (like Relevance Contrast or direct Spurious Perturbation), and the rationale for \carma{}'s specific choices are discussed in Appendix \ref{sec:causal_model_details}. 
% The combined dataset $\mathcal{D} = \mathcal{D}_{\mathrm{pref}} \cup \mathcal{D}_{\mathrm{causal}} \cup \mathcal{D}_{\mathrm{neutral}}$ (after filtering imperfect augmentations, see Section \ref{subsec:filtering_appendix}) provides the signal for robust training. The central idea is that explicit examples of disentanglement are key to teaching a reward model to distinguish causal quality drivers from spurious correlates. 
We provide the prompts for the generations described in Section \ref{sec:prompt_templates}.

==> archived/oc_20250515.tex <==
% \subsection{Our Contributions}
% \label{subsec:our_contributions}

The principal question we wish to address in the paper is the following:
\begin{remarkbox}{Mitigating Reward Hacking from Unknown Spurious Correlates via Causal Attributes}
How do we train reward models to be robust against reward hacking, particularly when the specific spurious attributes that an RM may exploit are not known a priori, by focussing only on stable causal drivers of answer quality found in ground truth/human preferences.
\end{remarkbox}


We provide the following main contributions in this work:
\textbf{1. Spurious-unaware Robustness} We introduce a causal framework (Section~\ref{sec:preliminaries}, Figure~\ref{fig:causal_graph}) that models answer generation by distinguishing fundamental \emph{causal} drivers of reward labels from \emph{spurious} correlates.


% We address the persistent challenge of \emph{reward hacking} in LLM alignment by proposing \textbf{\carma{} (Causal Augmentation to disentangle Reward Modeling Attributes)}. Our main contributions are:

% \vspace{-0.2in}
\begin{itemize}[left=2pt,itemsep=0pt]
    \item \textbf{A Principled Causal Framework for Spurious-Unaware Robust Reward Modeling.}
    We introduce a causal framework (Section~\ref{sec:preliminaries}, Figure~\ref{fig:causal_graph}) that models answer generation by distinguishing fundamental \emph{causal} drivers of reward labels from \emph{spurious} correlates. Crucially, this framework does not require a priori specification of spurious attributes, enabling \carma{} to train RMs that are robust to a broader range of unforeseen superficial cues while focusing on genuine quality.

    \item \textbf{Novel Targeted Augmentations for Causal and Neutral Attributes.}
    Building on our framework, we introduce \textit{targeted data augmentation for specific causal attributes} (Section~\ref{sec:methodology}). Unlike prior work focusing on broader neutral or coarse-grained augmentations, our \emph{Causal Augmentations} create minimal pairs isolating changes in individual causal dimensions (e.g., factuality, safety) to instill precise sensitivity. These are complemented by \emph{Neutral Augmentations} that enforce invariance to spurious features by varying them while preserving causal content, using tie-labels. We present a systematic generation and filtering process for these highly informative counterfactual examples. Our framework is also general enough to incorporate augmentation strategies from related works (Appendix \ref{sec:causal_model_details}). 
    {\color{blue} We query an oracle LLM to produce rubrics on a given answer that are only causally relevant to reward labeling and perform the above augmentations on those rubrics. We do not use any explicit knowledge of spurious factors/attributes.}
    \item \textbf{Formal Definition and Theoretical Guarantees for Reward Hacking Mitigation.}
    We provide a \textit{formal definition of spurious reward hacking} (Section~\ref{sec:theory}, Definition~\ref{def:reward_hacking_formal_theory} in Appendix~\ref{subsec:theory_definition}) and present a rigorous theoretical analysis. We prove that, under specified data coverage and optimization assumptions, an RM trained with \carma{}'s augmentation scheme is guided towards causal faithfulness and is robust against reward hacking via superficial manipulations (Theorem~\ref{thm:mitigation_formal_theory} in Appendix~\ref{subsec:theory_mitigation}).{\color{brown}: Can we move \emph{formal definition of reward hacking} to point no 1? Also do we really want to claim that we provide formal guarantees ? The empirical results are stronger compared to the theory so it is better to highlight that }

    \item \textbf{State-of-the-Art Empirical Performance and Downstream Alignment Benefits.}
    Comprehensive experiments (Section~\ref{sec:experiments}) demonstrate \carma{}'s superiority. On \textbf{RewardBench} \citep{lambert2024rewardbench}, \carma{} significantly outperforms standard RMs and strong baselines like \rrm{} \citep{liu2024rrm}, improving average accuracy by up to 5.4\%, with notable gains in Safety (up to \textbf{13.18\%}) and Reasoning (up to \textbf{7.19\%}) (Table~\ref{tab:performance_bt_pairpm_rewardbench}). We also beat the existing baselines on absolute robustness metric on \textbf{reWordBench} \citep{wu2025rewordbench}, which systematically transforms reward model inputs in meaning or ranking preserving ways (Figure \ref{fig:reword_absolute_robustness}). This robustness translates to downstream benefits: Best-of-N response selection using \carma{}-RMs improves AlpacaEval scores by up to 10\%, which is attributed to the \textit{diminished} reward hacking and enhanced performance.
\end{itemize}

==> archived/theory_20250506.tex <==

\section{Theoretical Analysis}
\label{sec:theory}

We provide a theoretical justification for why our data augmentation strategy mitigates reward hacking. The core idea is that by explicitly adding constraints related to causal and spurious attributes, we guide the learned reward model $\hat{R}_\phi$ to align more closely with the ground-truth reward structure $R^*$.

\subsection{Formal Setup}
We use the notation established in Section \ref{sec:preliminaries}. Key variables include the query $Q$, answer $A$, causal attributes $C(A)$, spurious attributes $SP(A)$, the ground-truth reward $R^*(Q, A) = f^*(Q, C(A))$, and the learned reward model $\hat{R}_\phi(Q, A)$. The training minimizes a combined loss $\mathcal{L}(\phi)$ (Eq. \ref{eq:combined_loss_methodology}) over the dataset $\mathcal{D} = \mathcal{D}_{hf} \cup \mathcal{D}_{aug}$.

\subsection{Definition of Spurious Reward Hacking}
We reiterate the formal definition for clarity.

\begin{definition}[Spurious Reward Hacking]
\label{def:reward_hacking_formal_simple}
A learned reward model $\hat{R}_\phi$ exhibits \emph{spurious reward hacking} if there exist $Q, A_{high}, A_{low}$ with $R^*(Q, A_{high}) > R^*(Q, A_{low})$, and $\tilde{A}_{low}$ such that $C(\tilde{A}_{low}) = C(A_{low})$, $SP(\tilde{A}_{low}) \neq SP(A_{low})$, but $\hat{R}_\phi(Q, \tilde{A}_{low}) > \hat{R}_\phi(Q, A_{high})$.
\end{definition}

\subsection{Impact of Augmented Data Constraints}

Our methodology introduces specific constraints via the augmented data $\mathcal{D}_{aug}$, which consists of causal pairs ($\mathcal{D}_{causal}$) and neutral pairs ($\mathcal{D}_{neutral}$). The combined loss function $\mathcal{L}(\phi)$ aims to satisfy these constraints.

\begin{proposition}[Neutral Constraint Encourages Spurious Invariance]
\label{prop:neutral_constraint}
The neutral loss term in $\mathcal{L}(\phi)$,
\[ \mathcal{L}_{tie}(\phi) = - \lambda \sum_{(Q, A_1, A_2, y=\text{tie})\in \mathcal{D}_{neutral}} [ \log \sigmoid(\Delta_{12}) + \log \sigmoid(-\Delta_{12}) ] \]
where $\Delta_{12} = \hat{R}_\phi(Q, A_1) - \hat{R}_\phi(Q, A_2)$, is minimized when $\hat{R}_\phi(Q, A_1) = \hat{R}_\phi(Q, A_2)$ for all neutral pairs $(A_1, A_2)$ in $\mathcal{D}_{neutral}$. By construction, neutral pairs aim to satisfy $C(A_1) = C(A_2)$ while $SP(A_1) \neq SP(A_2)$. Therefore, minimizing $\mathcal{L}_{tie}$ explicitly incentivizes the learned model $\hat{R}_\phi$ to be invariant to the specific spurious variations present in $\mathcal{D}_{neutral}$ when causal attributes are held constant.

\begin{proof}
The term inside the summation, $-[\log \sigmoid(\Delta_{12}) + \log \sigmoid(-\Delta_{12})]$, can be rewritten as $-[\log(P(A_1 \succ A_2)) + \log(P(A_2 \succ A_1))]$. This expression represents the negative log-likelihood of observing a tie under the Bradley-Terry model if we interpret a tie as equal probability for both outcomes. This loss is minimized when $P(A_1 \succ A_2) = P(A_2 \succ A_1) = 0.5$, which occurs precisely when $\Delta_{12} = \hat{R}_\phi(Q, A_1) - \hat{R}_\phi(Q, A_2) = 0$. Thus, the loss term drives $\hat{R}_\phi(Q, A_1) = \hat{R}_\phi(Q, A_2)$ for pairs designed to differ only in $SP$.
\end{proof}
\end{proposition}

\begin{proposition}[Causal Constraint Encourages Causal Sensitivity]
\label{prop:causal_constraint}
The standard preference loss term in $\mathcal{L}(\phi)$,
\[ \mathcal{L}_{pref}(\phi) = - \sum_{(Q, y_w, y_l) \in \mathcal{D}_{hf} \cup \mathcal{D}_{causal}} \log \sigmoid(\hat{R}_\phi(Q, y_w) - \hat{R}_\phi(Q, y_l)) \]
when applied to causal augmentation pairs $(y_w, y_l) \in \mathcal{D}_{causal}$, directly incentivizes the model $\hat{R}_\phi$ to assign higher scores to answers with improved causal attributes. Specifically, if $(A', A)$ is a causal pair constructed such that $A'$ is an improvement over $A$ only along causal attribute $C_j$ (i.e., $R^*(Q, A') > R^*(Q, A)$) and is labeled $A' \succ A$, minimizing the corresponding loss term $-\log \sigmoid(\hat{R}_\phi(Q, A') - \hat{R}_\phi(Q, A))$ encourages $\hat{R}_\phi(Q, A') > \hat{R}_\phi(Q, A)$.

\begin{proof}
The term $-\log \sigmoid(\Delta)$ is minimized as $\Delta \to \infty$. For a pair labeled $y_w \succ y_l$, the loss encourages the difference $\hat{R}_\phi(Q, y_w) - \hat{R}_\phi(Q, y_l)$ to be positive and large. When applied to causal pairs $(A', A)$ labeled $A' \succ A$ designed to isolate an improvement in a causal attribute $C_j$, this directly pushes the model to reflect that improvement with a higher score.
\end{proof}
\end{proposition}

\subsection{Mitigating Reward Hacking}

The combination of these two types of constraints directly counteracts the conditions required for spurious manipulation reward hacking.

\begin{theorem}[Mitigation of Spurious Manipulation Reward Hacking]
\label{thm:mitigation}
Training a reward model $\hat{R}_\phi$ by minimizing the combined loss $\mathcal{L}(\phi)$ (Eq. \ref{eq:combined_loss_methodology}) mitigates spurious manipulation reward hacking (Definition \ref{def:reward_hacking_formal_simple}). Specifically:
\begin{enumerate}
    \item The neutral loss term ($\mathcal{L}_{tie}$) penalizes differences in $\hat{R}_\phi$ arising solely from spurious attribute variations present in $\mathcal{D}_{neutral}$.
    \item The preference loss term ($\mathcal{L}_{pref}$) applied to $\mathcal{D}_{causal}$ rewards sensitivity to genuine causal attribute variations.
\end{enumerate}
Therefore, the optimization objective actively discourages the scenario where a spuriously modified answer $\tilde{A}_{low}$ (with $C(\tilde{A}_{low}) = C(A_{low})$) achieves a higher score than a causally superior answer $A_{high}$.

\begin{proof}
Consider the conditions for reward hacking: we need $\hat{R}_\phi(Q, \tilde{A}_{low}) > \hat{R}_\phi(Q, A_{high})$ despite $R^*(Q, A_{high}) > R^*(Q, A_{low})$ and $C(\tilde{A}_{low}) = C(A_{low})$.
Proposition \ref{prop:neutral_constraint} shows that the training objective encourages $\hat{R}_\phi(Q, \tilde{A}_{low}) \approx \hat{R}_\phi(Q, A_{low})$ if the specific spurious difference between $\tilde{A}_{low}$ and $A_{low}$ is covered by neutral pairs.
Proposition \ref{prop:causal_constraint} shows that the objective encourages $\hat{R}_\phi(Q, A_{high}) > \hat{R}_\phi(Q, A_{low})$ if the causal difference between $A_{high}$ and $A_{low}$ is covered by causal pairs.
Combining these, the objective encourages $\hat{R}_\phi(Q, A_{high}) > \hat{R}_\phi(Q, A_{low}) \approx \hat{R}_\phi(Q, \tilde{A}_{low})$. This directly opposes the inequality $\hat{R}_\phi(Q, \tilde{A}_{low}) > \hat{R}_\phi(Q, A_{high})$ required for reward hacking. The extent of mitigation depends on the coverage and quality of $\mathcal{D}_{aug}$ and the effectiveness of the optimization in satisfying the loss components.
\end{proof}
\end{theorem}

This analysis demonstrates that our proposed data augmentation strategy provides principled mechanisms for improving reward model robustness. The neutral augmentation specifically targets and penalizes reliance on spurious features by enforcing invariance, while the causal augmentation ensures sensitivity to genuine quality dimensions. Together, these components guide the learned reward model $\hat{R}_\phi$ towards the properties of the desired ground-truth reward $R^*$, thereby mitigating the potential for spurious manipulation reward hacking. 

\begin{rem}
The effectiveness in practice hinges on the quality of attribute identification and counterfactual generation, issues we investigate empirically in the upcoming Section \ref{sec:experiments}.    
\end{rem}



==> archived/theory_20250516.tex <==

We provide a high-level theoretical justification for \carma{}'s ability to mitigate spurious reward hacking, with full details and formal proofs deferred to Appendix \ref{sec:theoretical_analysis_detailed}. Our core argument is that by training with specifically constructed causal and neutral augmentation pairs, the learned reward model $\hat{\mathrm{R}}_\theta$ is guided away from relying on superficial correlations.

\vspace{-0.05in}
\subsection{Spurious Reward Hacking}
Consider three answers $\mathrm{A}_{high}$, $\mathrm{A}_{low}$, and $\tilde{\mathrm{A}}_{low}$ for a query $\mathrm{Q}$.
A reward model $\hat{\mathrm{R}}_\theta$ exhibits \textit{spurious reward hacking} if:
\begin{enumerate}[label=(\roman*), itemsep=0pt, left=15pt, topsep=3pt]
    \item $\mathrm{R}^*(\mathrm{Q}, \mathrm{A}_{high}) > \mathrm{R}^*(\mathrm{Q}, \mathrm{A}_{low})$ (causal superiority of $\mathrm{A}_{high}$ over $\mathrm{A}_{low}$),
    \item $\mathrm{C}(\tilde{\mathrm{A}}_{low}) = \mathrm{C}(\mathrm{A}_{low})$ and $\mathrm{SP}(\tilde{\mathrm{A}}_{low}) \neq \mathrm{SP}(\mathrm{A}_{low})$ (making $\tilde{\mathrm{A}}_{low}$ a spuriously modified version of $\mathrm{A}_{low}$, thus $\mathrm{R}^*(\mathrm{Q}, \tilde{\mathrm{A}}_{low}) = \mathrm{R}^*(\mathrm{Q}, \mathrm{A}_{low})$),
\end{enumerate}
\vspace{-0.05in}
yet the model $\hat{\mathrm{R}}_\theta$ prefers the spuriously modified inferior answer over the causally superior one:

\vspace{-0.15in}
\begin{equation}
\hat{\mathrm{R}}_\theta(\mathrm{Q}, \tilde{\mathrm{A}}_{low}) > \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_{high}).
% \text{Optionally, can also state: } \dots > \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_{low}) % if space and desired
\label{eq:hacking_condition_main}
\end{equation}
This captures exploitation via spurious manipulations. A formal definition is provided in Appendix \ref{subsec:theory_definition}. Using this definition, and assumptions on causal coverage, and model expressivity, we provide guarantees on mitigation of reward hacking. A formal statement and proof of Theorem \ref{thm:mitigation_main_informal} are provided in Appendix \ref{subsec:theory_mitigation}.

\vspace{-0.2in}
\subsection{Mitigation through Augmented Data Constraints}
\carma{}'s training objective (Eq. \ref{eq:combined_loss_methodology}) combines a standard preference loss with a tie-loss for neutral pairs. This structure, when applied to our augmented data, directly counteracts reward hacking.

\begin{theorem}[Mitigation of Spurious Reward Hacking (Informal)]
\label{thm:mitigation_main_informal}
Under specific assumptions about data coverage and optimization success (detailed in Appendix \ref{subsec:theory_assumptions}), training a reward model $\hat{\mathrm{R}}_\theta$ with \carma{}'s causally-informed data augmentation and composite loss discourages the model parameters $\theta$ from satisfying the spurious reward hacking condition (Eq. \ref{eq:hacking_condition_main}).
\end{theorem}

\vspace{-0.1in}
\paragraph{Intuition:}

\vspace{-0.05in}
\begin{enumerate}[itemsep=0pt, left=10pt, topsep=3pt]
    \item \textbf{Causal Sensitivity} from $\mathcal{D}_{\mathrm{causal}}$ encourages $\hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_{high}) > \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_{low})$.
    \item \textbf{Spurious Invariance} from $\mathcal{D}_{\mathrm{neutral}}$ encourages $\hat{\mathrm{R}}_\theta(\mathrm{Q}, \tilde{\mathrm{A}}_{low}) \approx \hat{\mathrm{R}}_\theta(\mathrm{Q}, \mathrm{A}_{low})$.
\end{enumerate}
These together guide $\hat{\mathrm{R}}_\theta$ towards $\hat{\mathrm{R}}_\theta(\mathrm{A}_{high}) > \hat{\mathrm{R}}_\theta(\mathrm{A}_{low}) \approx \hat{\mathrm{R}}_\theta(\tilde{\mathrm{A}}_{low})$, opposing the reward hacking condition. A formal statement and proof of Theorem \ref{thm:mitigation_main_informal} are provided in Appendix \ref{subsec:theory_mitigation}.
% Effectiveness depends on the quality of LLM-approximated counterfactuals.


